SmartOTPs: An Air-Gapped 2-Factor Authentication for Smart-Contract Wallets (Extended Version)

With the recent rise of cryptocurrencies' popularity, the security and management of crypto-tokens have become critical. We have witnessed many attacks on users and providers, which have resulted in significant financial losses. To remedy these issues, several wallet solutions have been proposed. However, these solutions often lack either essential security features, usability, or do not allow users to customize their spending rules. In this paper, we propose SmartOTPs, a smart-contract wallet framework that gives a flexible, usable, and secure way of managing crypto-tokens in a self-sovereign fashion. The proposed framework consists of four components (i.e., an authenticator, a client, a hardware wallet, and a smart contract), and it provides 2-factor authentication (2FA) performed in two stages of interaction with the blockchain. To the best of our knowledge, our framework is the first one that utilizes one-time passwords (OTPs) in the setting of the public blockchain. In SmartOTPs, the OTPs are aggregated by a Merkle tree and hash chains whereby for each authentication only a short OTP (e.g., 16B-long) is transferred from the authenticator to the client. Such a novel setting enables us to make a fully air-gapped authenticator by utilizing small QR codes or a few mnemonic words, while additionally offering resilience against quantum cryptanalysis. We have made a proof-of-concept based on the Ethereum platform. Our cost analysis shows that the average cost of a transfer operation is comparable to existing 2FA solutions using smart contracts with multi-signatures.

==> sec/analysis.tex <==
We analyze the security of SmartOTPs and its resilience to attacker models under the assumption of random oracle model $\mathcal{RO}$. % $\mathcal{RO}$ for $h(.)$.



\subsection{Security of OTPs}\label{sec:security-of-otps}
OTPs in our scheme are related to two cryptographic constructs: a list of hash chains and the Merkle tree aggregating their last values. 
%In the base version, only Merkle tree are presented while the full version contains both of these constructs.
%
%\subsubsection{Base Version}
%In the base version, only the Merkle tree is presented. 
%leaves of the Merkle tree (i.e., hashes of OTPs) are publicly known, therefore an adversary can launch an off-line attack to compute or ``collide with'' an unrevealed OTP (and thus breaking the second authentication factor).
%
%\subsubsection{Full Version}
In this subsection, we assume an adversary $\mathcal{A}$ who is trying to invert OTPs, and we give a concrete expressions for security of our scheme. 
%
%Our chain construction is motivated by T/Key proposed by Kogan et al.~\cite{kogan2017t}. 
Since we employ the hash domain separation technique~\cite{leighton1995large} for hash chains, each hash execution can be seen as an execution of an independent hash function.
%
For such a construction, Kogan et al. give the following upper bound (see Theorem 4.6 in~\cite{kogan2017t}) on the advantage of $\mathcal{A}$ breaking a chain:
\begin{eqnarray}\label{eqn:adv-breaks-single-chain}
Pr[\mathit{\mathcal{A}~breaks~a~chain}]\leq\frac{2Q+2P+1}{2^S},
\end{eqnarray}
where $Q$ is the number of queries that $\mathcal{A}$ can make to $h(.)$, $P$ is the chain length, and $S$ is the bit-length of OTPs (and the output of $h(.)$).  
%Thus, with a computationally bounded $\mathcal{A}$, who is able to make only a polynomial number of queries in $2^S$, this probability remains negligible.
Kogan et al.~\cite{kogan2017t} proved that inverting a hash chain hardened by the domain separation imposes a loss of security equal to the factor of 2.
Therefore, to make a hardened hash chain as secure as $\lambda\varDash{-} bit$ $\mathcal{RO}$, it is enough to set $S = \lambda + 2$.
%which means, according to the authors, that a hardened hash chain is as hard to invert as a single hash function.
E.g., to achieve 128-bit security, $S$ should be equal to 130.

\paragraph{SmartOTPs without Subtrees}
This scheme (see \autoref{subsec:caching-smart-contract}) uses a Merkle tree that aggregates $\mathcal{L}=\frac{N}{P}$ hash chains, where
the chains are created independently of each other; they have the same length and the same number of OTPs.
$\mathcal{A}$ can win by inverting any of the chains; hence, the probability that this scheme is secure is
%
\begin{eqnarray}\label{eqn:scheme-is-secure}
Pr[\mathit{Scheme~is~secure}] = \bigg(1-\frac{2Q+2P+1}{2^S}\bigg)^\mathcal{L}.
\end{eqnarray}
%
We can apply the alternative form of Bernoulli's inequality
$(1 - x)^\mathcal{L} \geq 1 - x\mathcal{L},$
where $\mathcal{L} \geq 1$ and $0 \leq x \leq 1$ must hold.
%
In our case, the input conditions hold since the number of hash chains is always greater than one and the probability that $\mathcal{A}$ breaks a single chain from \autoref{eqn:adv-breaks-single-chain} fits the range of $x$ (i.e.,  $0\leq\frac{2Q+2P+1}{2^S}\leq 1$).
%
Hence, we lower-bound the probability from \autoref{eqn:scheme-is-secure} as follows:
\begin{eqnarray}\label{eqn:scheme-is-secure-nosubtrees}
Pr[\mathit{Scheme~is~secure}] \geq 1 -\frac{\mathcal{L}(2Q+2P+1)}{2^S}.
\end{eqnarray}
%which with increasing $S$ is overwhelming.
%
\begin{corollary}
To make SmartOTPs without partitioning into subtrees as secure as $\lambda\varDash{-} bit$ $\mathcal{RO}$, it is enough to set $S = \lambda + 2 + log_2(\mathcal{L})$.
\end{corollary}
%which means, according to the authors, that a hardened hash chain is as hard to invert as a single hash function.
\noindent For example, to achieve 128-bit security with $\mathcal{L}=64$ and $P \geq 1$, $S$ should be equal to 136, and thus an OTP can be transferred by one QR code v1 or 13 mnemonic words.

\paragraph{Full SmartOTPs}
The full SmartOTPs scheme contains partitioning into subtrees, in which all leaves of the next subtree ``are visible'' only after depleting OTPs of the current subtree (and using OTPs from the 1st iteration layer of the next subtree). 
This improves the security of our scheme under the assumption that $\mathbb{C}$'s storage is not compromised by $\mathcal{A}$, which is true for $\mathcal{A}$ that possesses $PK_{\mathbb{U}}$ or~$\mathbb{A}$.
%
Therefore, we replace $\mathcal{L}$ in \autoref{eqn:scheme-is-secure-nosubtrees} for $\mathcal{L_S} = \frac{N_S}{P},$ $N_S \ll N$.
%\begin{eqnarray}\label{eqn:scheme-is-secure-full}
%Pr[\mathit{Scheme~is~secure}] \geq 1 -\frac{\mathcal{L_S}(2Q+2P+1)}{2^S},
%\end{eqnarray}
%
\begin{corollary}
	To make the full scheme of SmartOTPs as secure as $\lambda\varDash{-} bit$ $\mathcal{RO}$, it is enough to set $S = \lambda + 2 + log_2(\mathcal{L_S})$.
\end{corollary}
%
\noindent Therefore, to achieve 128-bit security with $\mathcal{L} = \frac{N}{N_S} \mathcal{L_S}$, $\mathcal{L_S}= 64$, and $P \geq 1$, $S$ should be equal to 136, and thus an OTP can be transferred by a QR code v1 or 13 mnemonic words.
To achieve the same security with $\mathcal{L_S}=1024$, we need to set $S= 140$, and thus an OTP can be transferred in a QR code v2 or 13 mnemonic words. 



\subsection{The Attacker Possessing $SK_{\mathbb{U}}$}

\begin{theorem}
%Requirements on OTPs:
$\mathcal{A}$ with access to $SK_{\mathbb{U}}$ is able to initiate operations by $\Pi_{O}$ but is unable to confirm them.
\end{theorem}

\vspace{-0.2cm}
\begin{proof1}
%Security of our scheme is achieved by meeting all requirements on OTPs (see \autoref{sec:design-space}) and by separating interaction with blockchain to two stages of protocol $\Pi_{O}$.
The security of $\Pi_{O}$ is achieved by meeting all requirements on general OTPs (see \autoref{sec:design-space}).
%
In detail, the requirement on the \textit{independence} of two different OTPs is satisfied by the definition of $F_k(.) \equiv h(k ~\|~ .)$, where $h(.)$ is instantiated by  $\mathcal{RO}$. 
This is applicable when $P=1$.
However, if $P>1$, then items in previous iteration layers of OTPs can be computed from the next ones.
Therefore, to enforce this requirement, we employ an explicit invalidation of OTPs belonging to all previous iteration layers by a sliding window at $\mathbb{S}$ (see \autoref{sec:increasingNoOfOTPs}).
%\psz{that probably, should be described somewhere before. It is security-critical and here we mention it first time. How do we invalidate it? A sliding window? Client obligated to kill it? Probably the former.}
%
The requirement on the \textit{linkage} of each $OTP_i$ with operation $O_i$ 
%in the current iteration layer 
is satisfied due to (1) $\mathcal{RO}$ used for instantiation of $h(.)$ and (2) by the definition of the Merkle tree, preserving the order of its aggregated leaves. 
%-- in particular the non-commutativity property of the concatenation, which enable us to unambiguously derive an index associated with an OTP using its proof.
%
By meeting these requirements, $\mathcal{A}$ is able to initiate an operation $O_j$ in the first stage of $\Pi_{O}$ but is unable to use an $OTP_i$ intercepted in the second stage of $\Pi_{O}$ to confirm $O_j$, where $j \neq i$.
%
Finally, the requirement on the \textit{authenticity} of OTPs is ensured by a random generation of $k$ and by anchoring $\mathcal{R}$ associated with $k$ at the constructor of $\mathbb{S}$.
\end{proof1}

\begin{theorem}
	Assuming $\delta \in \{0,\ldots, \frac{N}{N_S} - 2\}$, $\mathcal{A}$ with access to $SK_{\mathbb{U}}$ 
	%is able to deplete OTPs of the current (i.e., $\delta$th) subtree but 
	is unable to deplete all OTPs or misuse a stolen OTP that introduces the $(\delta + 1)$th subtree by $\Pi_{ST}$.
\end{theorem}

\vspace{-0.2cm}
\begin{proof1}
%First, we assume that $\delta \leq \frac{N}{N_S} - 2$.
When all but one OTPs of the $\delta$th subtree are depleted, the last remaining operation $O_{(N_S - 1) + \delta N_S}, ~\delta \in \{0, ~\ldots,~ \frac{N}{N_S} - 2\}$ is enforced by $\mathbb{S}$ to be the introduction of the next subtree. 
This operation is executed in a single transaction calling the function $nextSubtree()$ of $\mathbb{S}$ (see \autoref{alg:alg-next-child-tree}) requiring the corresponding $OTP_{(N_S - 1) + \delta N_S}$ that is under control of $\mathbb{U}$; hence $\mathcal{A}$ cannot execute the function to proceed with a further depletion of OTPs in the $(\delta + 1)th$ subtree. 
%, and at the same time, the consistency of the passed cached layer is verified against the parent $\mathcal{R}$.
If $\mathcal{A}$ were to intercept $OTP_{(N_S - 1) + \delta N_S}$ during the execution of $\Pi_{ST}$ by $\mathbb{U}$, he could use the intercepted OTP only for the introduction of the next valid subtree since the function $nextSubtree()$ also checks a valid cached sublayer of the $(\delta+1)$th subtree against the parent root hash $\mathcal{R}$.	
\end{proof1}	

\begin{theorem}
Assuming $\delta = \frac{N}{N_S} - 1$,
$\mathcal{A}$ with access to $SK_{\mathbb{U}}$ is neither able to deplete all OTPs nor introduce a new parent tree nor render SmartOTPs unusable. % when all but one operations are depleted.
\end{theorem}	

\vspace{-0.2cm}
\begin{proof1}
In contrast to the adjustment of the next subtree, the situation here is more difficult to handle, since the new parent tree cannot be verified at $\mathbb{S}$ against any paramount field. 
If we were to use $\Pi_{O}$ while constraining to the last initialized operation $O_{(N-1) + \eta N}, ~\eta \in \{0,1,\ldots\}$ of the parent tree, then $\mathcal{A}$ could render SmartOTPs unusable by submitting an arbitrary $\mathcal{R}$ in $initOp()$, thus blocking all the funds of the user.
If we were to allow repeated initialization of this operation, then we would create a race condition issue.
Therefore, this operation needs to be handled outside of the protocol $\Pi_{O}$, using two unlimited append-only lists $L_1$ and $L_2$ that are manipulated in three stages of interaction with the blockchain (see \autoref{sec:depletion-of-otps}).
%	, as described in \autoref{sec:depletion-of-otps}.
In the first stage, $h(\mathcal{R}^{new} ~\|~ OTP_{(N-1) + \eta N})$ is appended to $L_1$, hence $\mathcal{A}$ cannot extract the value of OTP.
In the second stage, $\mathcal{R}^{new}$ is appended to $L_2$,
and finally, in the third stage, the user reveals the OTP for confirmation of the first matching entries in both lists. 
%
Although $\mathcal{A}$ might use an intercepted OTP from the third stage for appending malicious arguments into $L_1$ and $L_2$, when he proceeds to the third stage and submits the intercepted OTP to $\mathbb{S}	$, the user's entries will match as the first ones. % and thus a benign $\mathcal{R}$ will be introduced. 
\end{proof1}


\subsection{The Attacker that Tampers with the Client}

\begin{theorem}
If $\mathbb{C}$ is tampered with after $\Pi_{B}$, $\mathbb{U}$ can detect such a situation and prevent any malicious operation from being initialized.
\end{theorem}	

\begin{proof1}
If we were to assume that $\mathbb{W}$ is implemented as a software wallet (or hardware wallet without a display), then $\mathcal{A}$ tampering with $\mathbb{C}$ might also tamper with the $\mathbb{W}$'s software running on the same machine. 
This would in turn enable a malicious operation to be initialized and further confirmed by $\mathbb{U}$, since $\mathbb{U}$ would be presented with a legitimate data in $\mathbb{C}$ and $\mathbb{W}$, while the transactions would contain malicious data.
%
Therefore, we require that $\mathbb{W}$ is implemented as a hardware wallet with a display, which exposes only signing capabilities, while $SK_{\mathbb{U}}$ never leaves the device (e.g., \cite{trezor-hw-wallet,keep-key,BitLox,ellipal-hw-wallet}).
Due to it, $\mathbb{U}$ can verify the details of a transaction being signed in $\mathbb{W}$ and confirm signing only if the details match the information shown in $\mathbb{C}$ (for $\Pi_{O}$) or $\mathbb{A}$ (for $\Pi_{NR}^{\mathcal{I}}$).	
%
We refer the reader to the work of Arapinis et al.~\cite{ArapinisGKK19} for the security analysis of hardware wallets with displays. % ...details of transactions being signed.
%
\end{proof1}


%\begin{theorem1}
%	If the client is tampered with after bootstrapping, and the next subtree needs to be introduced, $\mathcal{A}$ cannot misuse OTP to confirm a previously initialized but unconfirmed operation.
%\end{theorem1}	
%
%\begin{proof1}
%	If $\mathbb{U}$ accidentally initiates an operation with incorrect parameters,...
%	
%	
%
%	%
%	
%\end{proof1}


%\begin{theorem1}\label{theorem:Protocol_BS}
%	If the client is tampered with before an execution of  $\Pi_{B}^\mathcal{S}$, $\mathcal{A}$ can intercept $k$ but cannot spoof it.
%\end{theorem1}	
%
%\begin{proof1}
%	Although  $\Pi_{B}^\mathcal{S}$ assumes no attackers, as $k$ might be intercepted, we show that even in the case of assuming tampering with the client, $\mathcal{A}$ cannot get a full control over SmartOTPs or block the funds of the user.
%	%
%	During the bootstrapping, the user verifies the equality of $\mathcal{R}$ displayed in $\mathbb{W}$ with $\mathcal{R}$ displayed in $\mathbb{A}$.
%	This step disables $\mathcal{A}$ from spoofing $k$.\footnote{Note that without this step, $\mathcal{A}$ could spoof $k$ for $k'$, let the user to interact with SmartOTPs for some time (while pretending that OTPs from $\mathbb{A}$ work properly); then encrypt $k'$ and blackmail the user, asking for ransom to decrypt $k'$.}  
%	Next, it is straightforward to see that $\mathcal{A}$ holding $k$ cannot initiate any operation with SmartOPTs since he is not possessing $SK_{\mathbb{U}}$.
%\end{proof1}


\begin{theorem}
	If $\mathbb{C}$ is tampered with during an execution of  $\Pi_{B}^{\mathcal{I}}$, $\mathcal{A}$ can neither intercept $k$ nor forge $\mathcal{R}$ nor forge $PK_\mathbb{U}$.
\end{theorem}	

\vspace{-0.2cm}
\begin{proof1}
%	The following relates to the secure bootstrapping only (see \autoref{sec:base_version}). 
	When the protocol $\Pi_{B}^{\mathcal{I}}$ is used, instead of an air-gapped transfer of $k$ from $\mathbb{A}$ to $\mathbb{C}$, $\mathbb{U}$ transfers leaves of the Merkle tree by microSD card.
	The leaves represent hashes of OTPs in the base version or the hashes of the last items of hash chains in the full version of SmartOTPs.  
	In both versions, the transferred data do not contain any secrets, hence $\mathcal{A}$ cannot take advantage of intercepting them.
	The next option that $\mathcal{A}$ may seek for is to forge $\mathcal{R}$ for $\mathcal{R}'$ and $PK_\mathbb{U}$ for $PK_\mathcal{A}$, which results in different $\mathbb{S}^{ID}$ than in the case of $\mathcal{R}$ and $PK_\mathbb{U}$, since $\mathbb{S}^{ID}$ is computed as $h(PK_\mathbb{U} ~\|~ \mathcal{R})$.
%	 and thus each pair of public key and root hash maps to the only $\mathbb{S}^{ID}$.
	%
	While $PK_\mathbb{U}$ is stored at $\mathbb{W}$, the authenticity of $\mathcal{R}$ needs to be verified by $\mathbb{U}$ who compares displays of $\mathbb{A}$ and $\mathbb{W}$.
	Only in the case of equality, $\mathbb{U}$ knows that $\mathbb{S}^{ID}$ displayed in $\mathbb{W}$ maps to legitimate $PK_\mathbb{U}$ and $\mathcal{R}$.
	%
\end{proof1}




\subsection{The Attacker Possessing the Authenticator}
It is trivial to see that $\mathcal{A}$ with access to $\mathbb{A}$ is unable to initialize any operation with SmartOTPs since he does not hold $PK_\mathbb{U}$. % required for initialization of operations.
%This property is inherited from general 2FA schemes that use OTPs.


\subsection{Further Properties and Implications}

\paragraph{\textbf{Requirement on Block Confirmations}}
Most cryptocurrencies suffer from long time to finality, potentially enabling the accidental forks, which create parallel inconsistent blockchain views.
On the other hand, this issue is not present at blockchain platforms with fast finality, such as Algorand~\cite{gilad2017algorand}, HoneyBadgerBFT~\cite{miller2016honey}, or StrongChain~\cite{strongchain}. % enabling the direct application of SmartOTPs.
%
In blockchains with long time to finality, overly fast confirmation of an operation may be dangerous, as, if an operation were initiated in an ``incorrect'' view, an attacker holding $SK_{\mathbb{U}}$ would hijack the OTP and reuse it for a malicious operation settled in the ``correct'' view. 
%
To prevent this threat, the recommendation is to wait for several block confirmations to ensure that an accidental fork has not happened. 
For example, in Ethereum, the recommended number of block confirmations to wait is 12 (i.e., $\sim$3 minutes).
Note that such waiting can be done as a background task of $\mathbb{C}$, hence $\mathbb{U}$ does not have to wait: 
(1) considering that $\mathcal{A}$ possesses $SK_{\mathbb{U}}$, $\mathbb{C}$ can detect such a fork during the wait and resubmit the $initOp()$ transaction, 
(2) in the case of $\mathcal{A}$ tampering with $\mathbb{C}$, no operation can be initialized since $\mathbb{U}$ never signs $\mathcal{A}$'s transaction (due to the hardware wallet), and 
(3) $\mathcal{A}$ possessing $\mathbb{A}$ cannot initialize any operation as well. 
%
% We stress that for our protocol it is crucial to wait such a recommended number of block confirmations before submission of a confirmation transaction, and thus ensure that an initialization transaction cannot be reversed.\footnote{The same apply for first two stages when introducing a new root hash.}
% Nevertheless, such a waiting can be implemented at the client, hence a user would not have to wait.

\paragraph{Attacks with a Post Quantum Computer}
Although a resilience to quantum computing (QC) is not the focus of this paper, it is of worthy to note that our scheme inherits a resilience to $QC$ from the hash-based cryptography.
% 
The resilience of our scheme to QC is dependent on the output size of $h(.)$. % and thus a bit length of OTPs.
A generic QC attack against $h(.)$ is Grover's algorithm~\cite{grover1996fast}, providing a quadratic speedup in searching for the input of the black box function.
%
%Nevertheless, early quantum computers are likely to have limited depth, and thus direct application of Grover's algorithm is likely to be infeasible~\cite{abdalla2016algorithms}.
%
As indicated by Amy et al.~\cite{amy2016estimating}, using this algorithm under realistic assumptions, the security of SHA-3 is reduced from 256 to 166 bits.
Applying these results to OTPs with 128-bit security from examples in \autoref{sec:security-of-otps}, we obtain 98-bits post-QC security. % which provides near term security (i.e., 10 years). 
Further, when assuming the example with $\mathcal{L}=64$ from \autoref{sec:security-of-otps} and~\cite{amy2016estimating}, to achieve 128-bits of post-QC security, we estimate the length of OTPs to 205-bits.

%\ih{From review A: "One question that would be helpful to address is whether or not the length of the OTPs need to increase to provide 128-bits of post-quantum security i.e., considering attacks like Grover's algorithm."}

%
%Note that with progress in QC, parameters of our system can be readjusted.
%\todo{We applied this methodology to various sizes of OTPs (see Appendix X) and found out that the size of OTPs in our scheme can be decreased even to $12B$ to improve its usability.} %, while still preserving near term security guarantees.}
% which may apply to the shrunk version of SHA-3 as well.
%Nevertheless, with regards to the current quantum computing power, the size of OTPs in our scheme can be decreased to $12B$ to improve usability.
%ECRYPT-2018:
% "In practice early quantum computers are likely to be of limited depth, and hence a direct application of Grovers’ algorithm to symmetric key search is likelyto be infeasible." 



==> sec/conclusion.tex <==
In this paper, we have proposed SmartOTPs, a smart-contract wallet framework that provides a secure and usable method of managing crypto-tokens.
% in an air-gapped setting. % in a self-sovereign fashion.
The framework provides 2FA that is executed in two stages of interaction with the blockchain and protects against the attacker possessing a user's private key or a user's authenticator or the attacker that tampers with the client.
%
Our framework uses OTPs constructed using 
%standard cryptography constructs, namely 
a pseudo-random function, Merkle trees, and hash chains.
We combine these primitives in a novel way, which enables an air-gapped setting using transcription of mnemonic words or scanning of small QR codes. % that protects against a Man-in-the-Machine~\cite{bui2018man} attacker as well as quantum computer attacks.
The protocol of our framework is general and can be utilized, besides the wallets, in any smart contract application for the purpose of 2FA. 
The provided smart contract is self-contained but its operation set can be extended by the community.
%
%We implemented our approach, basing on the Ethereum cryptocurrency and the Solidity language. 
%We performed a cost analysis of the implementation, showing that an average cost of a transfer operation is about $\$0.5$. 
%
% In the future work, we plan to add new operations to the smart contract, especially appending a new root hash before OTPs are depleted, which enables a user to stay at the same address when this happen. 
% As the next improvement, we plan to make our approach more cost efficient at the side of the smart contract by utilizing other operations than concatenation for implementation of a Merkle tree.
%In particular, we  resolved time-space tradeoff
%We have implemented our scheme and deployed it in a real-world scenario. 
%Our analysis and performance results show its feasibility and efficiency.
%
%In future work, we plan to investigate 2FA schemes in the context of emerging privacy-preserving smart contract platforms~\cite{kosba2016hawk},~\cite{cheng2018ekiden}.



%\section*{Acknowledgment} 
%This research was partially supported by ST Electronics and National Research Foundation (NRF), Prime Minister's Office Singapore, under Corporate Laboratory @ University Scheme (Programme Title: STEE Infosec -- SUTD Corporate Laboratory).
%%
%Also, the work was partially supported by the H2020 ECSEL project Aquas (8A17001), the IT4Innovations Excellence in Science project LQ1602, and the internal project of Brno University of Technology number FIT-S-17-4014. 


==> sec/costs.tex <==


Executing smart contracts over blockchain, i.e., performing computations and storing data, has its costs. 
In Ethereum Virtual Machine (EVM), these costs are expressed by the level of execution complexity of particular instructions, referred to as \textit{gas}.
One unit of gas has its market price in GWEI.
%
In this section, we analyze the costs of our approach using the same bit-length $S$ for $h(.)$ as well as for OTPs.
%
$S$ significantly influences the gas consumption for storing the cached layer on the blockchain. % while the effect of $O$ is negligible.
%
We remark that measured costs can also be influenced by EVM internals (e.g., 32B-long words/alignment).
%One such a mechanism is a 32B-long alignment of data fields and contract codes.
%
% there is a scheme-agnostic factor that influences the deployment and the operational costs of the smart contract.
% This factor stands for the memory alignment of the data fields in the smart contract's code and in its data structures. 
%  the case of EVM, the alignment should respect the block size equal to 32B. 
% If this is respected, then all storage and operational costs can be minimized.
%
% \ih{drop}
%In the following, we perform a series of gas measurements experiments investigating the parameters of the Merkle tree and hash chains.
%
%


%\vspace{-0.3cm}
\subsubsection{\textbf{Costs Related to the Merkle Tree}}\label{sec:costs-MK}
\hfill

\paragraph{\textbf{Deployment Cost}}
The cost of a smart contract deployment is driven mainly by the $L_S$ (related to the first subtree) and $S$. % of each hash in this sublayer.
%
A less significant factor is the consistency check of a Merkle tree, which is driven by $L_S$: 
%which first computes the root hash of the first subtree from the cached sublayer
%\footnote{i.e., See  \textit{reduceMT()} from \autoref{alg:MT-reduce-root} in Appendix.} 
%and then verifies the consistency of the subtree against the parent root hash.  
%(i.e., \textit{checkSubtreeConsistency()}).
the higher $L_S$ is, more layers have to be reduced.
Similarly, the greater $H-H_S$ is, more steps have to be done in the proof verification.
On the other hand, deployment costs are independent of the length $P$ of a hash chain; therefore, we omit the hash chain in this experiment and set $P=1$.
%\psz{current measurements?}
%
Further, we abstract from the concept of subtrees in order to analyze a single tree (i.e., $H = H_S$).
%
The deployment costs of our scheme with respect to the depth $L$ ($\equiv L_S$) of the cached layer are presented in \autoref{fig:MT-deploy-costs}.
The figure depicts two cases: one uses a single $\mathbb{S}$ and the second assumes a contract factory producing instances of $\mathbb{S}$.
Thanks to the contract factory, we managed to save a constant amount of  gas equal to $\sim1.3M$, regardless of $L_S$.
%\db{save when $L_S = 7$?}.\ih{it does not relate}
%
Since we assume $8M$ as the maximum gas limit at the Ethereum main network, we can build a caching layer with $L_S=7$ at maximum. % (i.e., requiring $6.6M$ of gas for deployment). 
Later, we will see that the maximum $H_S$ that can be used for the optimal caching layer of a subtree is $H_S = 10$, yielding $2^{10}$ leaves and thus $2^{10} P$ OTPs per subtree.
%Note that $N$ does not influence the deployment costs but operational costs, therefore we omit this parameter here.
%\psz{it really does not influence the deploy cost?}


\begin{figure}[t]
	\begin{center}		
		%				\vspace{-0.8cm}
		\includegraphics[width=0.39\textwidth]{fig/deployment-costs.pdf} 
		\vspace{-0.3cm}
		\caption{Deployment costs ($H = H_S$).}
		\label{fig:MT-deploy-costs}
		\vspace{-0.1cm}
	\end{center}	
\end{figure}


\paragraph{\textbf{Cost of a Transfer}}
Although the cost of each operation supported by $\Pi_{O}$ is similar, here we selected the transfer of crypto-tokens $O^t$, 
and we measured the total cost of $O^t$ as follows: 
%
\vspace{-0.1cm}
\medmuskip=0mu\thinmuskip=0mu\thickmuskip=-0mu
\begin{eqnarray*}
	O^t\_cost(L, ~N, ~P)&=&  
	  \overline{cost} \left(O^t(L, ~N, ~P) \right)
			    +  \frac{cost \left(O^d(L) \right)}{N}, \\
	\overline{cost} \left( O^t(L, ~N, ~P) \right) &=& \frac{1}{N} \sum_{i=1}^{N}{ cost \left(O^{t}_{i}(L, ~N, ~P) \right)},  \\
	cost \left(O^{t}_{i}(L, ~N, ~P) \right) &=& cost \left( O^{t.init}_i \right) + cost \left( O^{t.confirm}_i(L, ~N, ~P) \right),
\end{eqnarray*}
\medmuskip=3mu\thinmuskip=1mu\thickmuskip=5mu
%
where \textit{cost()} measures the cost of an operation in gas units, and $O_d$ represents the deployment operation.
%, $N$ represents the number of all transfers, $L$ the depth of the cached layer, and $P$ the size of hash chain.
%
As the purpose of the cached layer is to reduce the number of hash computations in \textit{confirmOp()}, the size of an optimal cached layer is subject to a trade-off between the cost of storing the cached layer on the blockchain and the savings benefit of the caching.
%
To explore the properties of the only Merkle tree, we adjusted $H = H_S$ and $P = 1$.
As each execution of $O^t$ (i.e., $O^t_i$) may have a slightly different gas cost, we measured the average cost of a transaction (i.e., $\overline{cost}(O^t(L, ~N, ~P)$) for both stages of $\Pi_{O}$; note that the cost of $initOp() \simeq 70k$ of gas in all operations.
%\footnote{Notice that this spread is small and is caused by different left/right positions of items in authentication paths of various leafs. The spread becomes more significant in the case of $P ~>~ 1$.}
%
For completeness, we present the transaction costs of all proposed operations in Appendix~\ref{appendix:cost-of-all-operations}.
%.
%
% We can see that the bigger is the number of OTPs, the lesser is the total average cost per transfer.
In \autoref{fig:MT-expenses}, we can see that the total average cost per transfer decreases with the increasing number of OTPs, as the deployment cost is spread across more OTPs.
%
%For each $N$, we highlight the optimal point that represents the depth of the cached layer for which the total cost per transfer is minimized.
The optimal point depicted in the figure minimizes $O^t$ by balancing $cost(O^d(L))$) and  $\overline{cost}(O^t(L, ~N, ~P))$.
We see that $L=H-3$ for such an optimal point.
%
In contrast to the version without caching, this optimization has brought a cost reduction of $3.87\%, ~5.61\%, ~7.32\%, ~\text{and} ~8.92\%$, for $128$, $256$, $512$, and $1,024$ leaves, respectively.
%
Next, we explored the number of transfer operations to be executed until a profit of the caching has begun (see \autoref{fig:MT-current-benefit-of-caching}).
We computed a rolling average cost per $O^t$, while distinguishing between the optimal caching layer and disabled caching % (i.e., $L = 0$).
-- the profit from caching begins after $53$, $90$, and $156$ transfers, respectively.
%The tipping point that marks the beginning of a profit from caching is at $53$, $90$, and $156$ transfers for $H$ equal $8$, $9$, and $10$, respectively.


\paragraph{\textbf{Costs with Subtrees}}
We measured the cost of introducing the next subtree within a parent tree depending on $L_S$, while we set $H = 20$ and $H_S = 10$ (see \autoref{fig:cost-of-new-subtree}).
We found out that when subtrees (and their cached sublayers) are introduced within a dedicated operation, it is significantly cheaper compared to the introduction of a subtree during the deployment.
%
%Thanks to this finding, we can further decrease the average total cost per operation, and moreover we can cache sublayers up to the depth of $9$.
%With this in mind, we calculate an average cost per transfer at $136,042$ of gas, which is $26\%$ less than in the case without subtrees and caching.
%

%\subsubsection{\textbf{Signing Schemes}}
%
%\paragraph{\textbf{Deployment Cost}}
%The cost of the signing schemes is influenced only by a size of a smart contract itself and storing of the minimal information required to provide contract functionality. 
%In contrast to the Merkle Tree schemes, here we save deployment costs due to the following reasons: 
%1) the authenticator's public key always contains only a single address field, thus no caching is possible here, 
%2) no buffer and its clearing mechanism is required,
%and 3) no consistency checks are required.
%%
%These differences cause the deployment costs to be $2,075,490$ in the case of signing operation ID and $1,906,361$ in the case of signing the whole transaction.
%
%
%\paragraph{\textbf{Total Expenses per Transfer}}
%Similarly as in the case of the Merkle tree scheme, here we also quantified the total expenses of a transfer operation with regards to the deployment cost and the number of expected confirmation materials, while we used the same measurement approach and the formula.
%%
%The total expenses per a transfer operation with various gas prices (i.e., value $K$) are depicted in \autoref{fig:Signing-expenses}.
%We can see that more operations a user intends to perform, the lower are total expenses per a transfer. 
%However, let us remark that in contrast to the Merkle tree scheme, here the number of expected operations does not need to be calculated beforehand.
%If the number of expected operations is over $4096$, then one may omit saving at the deployment stage of the contract and adjust $K = 1$.
%%
%We also observe that more optimal cost of the transfer operation was achieved in the case of signing the whole transaction than in the case of signing the operation ID.
%This is explained due to implicit recovery of public key (and its address) from a signed transaction, which is performed for free by the infrastructure of Ethereum.
%While in the case of signing operation ID, the explicit recovery of the public key has to be performed inside of the smart contract.
%%
%\begin{figure}
%	\centering
%	
%	\subfloat[\label{fig:sign-OpID-expenses}Signing operation IDs]{
%		\includegraphics[width=0.24\textwidth]{fig/expenses-OpID-crop.pdf} 
%		\vspace{0.5em} 
%	}
%	\subfloat[\label{fig:sign-TX-expenses}Signing whole transactions]{
%		\includegraphics[width=0.24\textwidth]{fig/expenses-TX-crop.pdf} 
%		\vspace{0.5em} 
%	}
%	
%	\caption{Total expenses per single transfer operation of signing scheme, while considering different ratio $K$ for saving the deployment cost.}
%	\label{fig:Signing-expenses}
%\end{figure}
%
%\paragraph{\textbf{Costs of All Operations}}
%Costs related to all implemented operations of the signing schemes are shown in the first two columns of \autoref{tab:other-costs}.
%Deployment costs are not assumed in this table, and thus it contains only instant cost of transaction calls.
%%
%The lower expenses per each type of operation are achieved in the case of signing the whole transaction in contrast to signing only operation ID due the same reason as above.

\begin{figure}[t]
	\centering
	\vspace{-0.3cm}
	\includegraphics[width=0.35\textwidth]{fig/expenses-Merkle-Tree-B16.pdf} 
	
	\vspace{-0.2cm}
	\caption{Average total cost per transfer ($H = H_S$).}\label{fig:MT-expenses}
	%	\vspace{0.2cm}
\end{figure}


\subsubsection{\textbf{Costs Related to Hash Chains}}
Since each iteration layer of hash chains contributes to an average cost of $confirmOp()$ with around the same value, we measured this value on a few trees with $P$ up to 512. % and found out that it is equal, on average, to $170$ units of gas.
%
Next, using this value and the deployment cost, we calculated the average total cost per transfer by adding layers of hash chains to a tree with $H = H_S$, thus increasing $N$ by a factor of $P$ until the minimum cost was found.
%
As a result, the optimal caching layer shifted to the leaves of the tree (see \autoref{fig:expenses-hash-chain-optim}), which would however, exceed the gas limit of Ethereum.
To respect the gas limit, we adjusted $L = 7$, as depicted in \autoref{fig:expenses-hash-chain-maxCache}.
%In such a setting we achieved the biggest saving for a tree with $H = 7$, while with a bigger $H$, the saving decreases.
%
In contrast to the configurations with $L = 0~\text{and}~ P = 1$ (from \autoref{fig:MT-expenses}), we achieved savings of $27.80\%$, $19.61\%$, $14.95\%$, and $12.51\%$ for trees with $H$ equal to $7$, $8$, $9$, and $10$, respectively.
%
For completeness, we calculated costs for $L=0$ as well (see \autoref{fig:expenses-hash-chain-zero-cache}).
%
Note that for $L = 0$ and $L = 7$, smaller trees are ``less expensive,'' as they require less operations related to the proof verification in contrast to bigger trees; these operations consume substantially more gas than operations related to hash chains.
%
Although we minimized the total cost per transfer by finding an optimal $P$, we highlight that increasing $P$ contributes to the cost only minimally but on the other hand, it increases the variance of the cost.
Hence, one may set this parameter even at higher values, depending on the use case.
% depending on the use case.


%\vspace{-0.2cm}
\subsubsection{\textbf{Costs in Fiat Money}}\label{sec:fiat-money}
We assume the average exchange rate of ETH/USD equal to $211$ and the ``standard'' gas price $5$ GWEI
%\footnote{\url{https://ethgasstation.info/}.} 
as of May 2, 2020.
%
For example, in the case of $N = 2^{25}$ (i.e., $H = 20, ~H_S = 10, ~P = 2^{5}, ~L_S=7 $), expenses per transfer operation are $\$0.2$, while expenses for deployment and introduction of a new subtree are $\$6.90$ and $\$1.23$, respectively.

%We assume the average exchange rate of ETH/USD equal to $147$ and the ``standard'' gas price $4$ GWEI
%%\footnote{\url{https://ethgasstation.info/}.} 
%as of December 1, 2019.
%%
%For example, in the case of $N = 2^{25}$ (i.e., $H = 20, ~H_S = 10, ~P = 2^{5}, ~L_S=7 $), expenses per transfer operation are $\$0.11$, while expenses for deployment and introduction of a new subtree are $\$3.85$ and $\$0.69$, respectively.
%%With $P = 2^{10}$, expenses per transfer are $\$0.15$.




==> sec/details.tex <==
\subsection{Increasing the Number of OTPs}\label{sec:increasingNoOfOTPs}
%
A small number of OTPs can have negative usability and security implications.
First, users executing many transactions\footnote{E.g., several smart contracts in Ethereum have over $2^{20}$ transactions made.}
would need to create new
OTPs often, and thus change their addresses.
%
Second, an attacker possessing $SK_{\mathbb{U}}$ can flood $\mathbb{S}$ with initialized operations, rendering all the OTPs unusable.
Therefore, we need to increase the number of OTPs to make the attack unfeasible.
%
However,  increasing the number of OTPs linearly increases the amount of data
that $\mathbb{C}$ needs to preserve in its storage. % (i.e., leaves of the tree or all nodes of the tree).
%
For example, if the number of OTPs is $2^{20}$, then $\mathbb{C}$ has to
store $33.6MB$ of data (considering $S=16B$ and $\mathbb{C}$ storing all leaves), which is feasible even on storage-limited devices.
However, e.g., for $2^{32}$ OTPs, $\mathbb{C}$ needs to store $137.4GB$ of data, which might be infeasible even on PCs, especially when $\mathbb{C}$ handles multiple instances of SmartOTPs.

To resolve this issue, we modify the base approach by applying a
time-space trade-off~\cite{hellman1980cryptanalytic} for OTPs.
Namely, we introduce  hash chains of which last items are aggregated by the Merkle tree. 
With such a construction, OTPs can be encoded as elements of chains and revealed layer by layer in the reverse order of creating the chains. 
This allows multiplication of the number of OTPs by the chain length without
increasing the $\mathbb{C}$'s storage but imposing a larger number of hash computations on $\mathbb{S}$ and $\mathbb{A}$.
Nonetheless, smart contract platforms set only a low execution cost for $h(.)$.

%
An illustration of this construction is presented in the bottom left part of
\autoref{fig:overview}.\footnote{Note that this figure contains further, not yet
described, improvements.}
A hash chain of length $P$ is built from each OTP assumed so far. 
Then, the last items of all hash chains are used as the first iteration layer, which provides $\frac{N}{P}$ OTPs.\footnote{For simplicity, we assume  that $GCD(N,P) = P$.} 
Similarly, the penultimate items of all the hash chains are used as the second iteration layer, etc., until the last iteration layer consisting of the first items of hash chains (i.e., outputs of $F_k(.)$) has been reached (see the middle part of \autoref{fig:overview}).
%
We emphasize that introducing hash chains may cause a violation of the requirement on the independence of OTPs if implemented incorrectly; 
i.e., OTPs from upper iteration layers can be derived from lower layers.
Therefore, to enforce this requirement, we invalidate all the OTPs of all the previous iteration layers by a sliding window at $\mathbb{S}$.

Furthermore, if a hash chain were to use the same hash function throughout the entire chain, it would be vulnerable to birthday attacks~\cite{hu2005efficient}.
%
To harden a hash chain against a birthday attack, a \textit{domain separation} proposed by Leighton and Micali~\cite{leighton1995large} can be used: a different hash function is applied in each step of a hash chain.
Note that without domain separation, inverting the $i$th iterate of $h(.)$ is $i$ times easier than inverting a single hash function (see the proof in~\cite{haastad2001practical}).
%
Therefore, we use a different hash function for all but the last iteration layer $1 \leq i < P$ as follows:
%\footnote{The last iteration layer is computed by $F_k(.)$}
\begin{eqnarray}\label{eqn:hash-with-domain-sep}
h_{\mathcal{D}[i]}(x) &=& h(P - i + 1~||~x),
\end{eqnarray}
where $x$ represents the OTP from the next iteration layer.
%\footnote{Note that this function is an inversion of function ...}

Although domain separation hardens a single hash chain against the birthday attack, this attack is still possible within the current iteration layer, which is an inevitable consequence of using multiple hash chains.
Therefore, the number of leaves $\mathcal{L}$ (i.e., N/P) is the parameter that must be considered when quantifying the security level of our scheme (see \autoref{sec:analysis}). 


With this improvement, $\mathbb{A}$ is updated to provide OTPs by
%
\begin{eqnarray}\label{eqn:hash-chains}
	getOTP(i) &=& h^{\alpha(i)}_{\mathcal{D}} \Bigg( F_k \Big(\beta(i) \Big) \Bigg),
%	\alpha(i) &=& P - \left\lfloor  \frac{i P}{N} \right\rfloor - 1, \\
%	\beta(i) &=& i ~\%~ \frac{N}{P},   
\end{eqnarray}
%
where $i$ is the operation ID, $\alpha(i)$ determines the index in a hash chain, 
%(i.e., a number of hash computations)
and $\beta(i)$ determines the index in the last iteration layer of OTPs.
% (i.e., outputs of pseudo-random function).
We provide concrete expressions for $\alpha(i)$ and $\beta(i)$ in \autoref{eqn:alpha-beta-final}, which involves all proposed improvements and optimizations.
%
A derivation of $\mathcal{R}$ from the OTP at $\mathbb{S}$ needs to be updated as well (see \autoref{alg:MT-deriveRH-hash-chains} in Appendix).
%\footnote{Note that the algorithm contains further, not yet described, improvements.}
In detail, $\mathbb{S}$ executes $P ~-~ \alpha(i) ~-~ 1 = \left\lfloor \frac{i P}{N} \right\rfloor$ hash computations, which is a complementary number to the number of hash computations at $\mathbb{A}$ with regard to $P$.
%
Also, $\mathbb{C}$ has to be modified, requiring computation of a proof to use the leaf index relative to the current iteration layer of OTPs (i.e., $i ~\%~ \frac{N}{P})$.
%

With this improvement, given the number of leaves equal to $2^{20}$ and $P=2^{12}$, $\mathbb{C}$ stores only $33.6MB$ of data and it has $2^{32}$ OTPs available.
%
On the other hand, this modification implies, on average, the execution of additional $P/2$ hash computations  at $\mathbb{S}$, imposing additional costs.
However, our experiments show the benefits of this approach (see \autoref{sec:costs-analysis}). 
%Also, note that with hash chains the lowest cost of operations occurs for the first iteration layer, while the highest cost occurs for the last iteration layer; hence even if user would not deplete all operation
%


\begin{figure*}[t]
	\begin{center}
		\vspace{-0.5cm}
		\includegraphics[width=0.98\textwidth]{fig/overview-tmp.pdf} 
		\vspace{-0.4cm}
		\caption{An overview of our approach and its improvements.
			%
			%		In the left part of the figure, we depict the partitioning of a tree into subtrees. 
			%		For each subtree we append hash chains that balance the size of the client's storage and the number of hash computations at the smart contract.
			%		%
			%		In the middle part of the figure, we depict the adjustment of the next parent tree.
			%		%
			%		In the right part of the figure, we depict the details of a subtree, which contains a split control in the provision/verification of OTPs (and their proofs) across the components of our framework.
			%		% Following are just details. Maybe drop.	
			%		In detail, OTPs are provided by the authenticator, while proofs are constructed from the $H$th layer of the parent Merkle tree stored at the client. 
			%		A proof contains only $H_S - L_S$ nodes, as the remaining  $L_S$ nodes are under the control of the smart contract.
		}
		\label{fig:overview}
		\vspace{-0.3cm}
	\end{center}	
\end{figure*}


\begin{algorithm}[!b]
	\footnotesize
	
	\SetKwProg{func}{function}{}{}
	
	$L_1$ $\leftarrow$ []; \Comment{Items have form $<h(\mathcal{R}^{new} ~\|~ OTP)>$}\\
	$L_2$ $\leftarrow$ []; \Comment{Items have form $<$ $\mathcal{R}^{new}$$>$}\\
	
	\smallskip
	\func{$1\_newRootHash$(hRootAndOTP) \textbf{public}}{
		\textbf{assert} $\Sigma.verify(tx.\sigma, PK_\mathbb{U})$;\\
		\textbf{assert} $nextOpID ~\%~ N = N - 1$; \Comment{The last oper. of tree} \\
		$L_1$.append(hRootAndOTP); \\
	}					
	
	%	\smallskip
	\func{$2\_newRootHash$($\mathcal{R}^{new}$) \textbf{public}}{
		\textbf{assert} $\Sigma.verify(tx.\sigma, PK_\mathbb{U})$;\\
		\textbf{assert} nextOpID$~\%~N = N - 1$; \Comment{The last oper. of tree}\\
		$L_2$.append($\mathcal{R}^{new}$);\\
	}
	
	%	\smallskip
	\func{$3\_newRootHash$(otp, $\pi$) \textbf{public}}{
		%		\textbf{assert} \textit{sender} = owner; \\
		\textbf{assert} nextOpID$~\%~N = N - 1$; \Comment{The last oper. of tree} \\
		verifyOTP(otp, $\pi$, nextOpID); \\
		\If{$L_1\text{.len} > LEN_{MAX} ~|~ L_2\text{.len} > LEN_{MAX}$}{			
			$L_1$, $L_2$ $\leftarrow$ [], []; \\
			\textbf{return}; \Comment{To avoid $\mathcal{A}$ DoS-ing $\mathbb{S}$ by gas depletion.} \\
		}
		\For{$\{i \leftarrow 0; ~i < L_2\text{.len} ; ~i\texttt{++}\}$}{
			\For{$\{j \leftarrow 0; ~j < L_1\text{.len} ; ~j\texttt{++}\}$}{
				\If{h($L_2$[i] $\|$ otp) = $L_1$[j]}{
					% reinitTree(list2[i], $childLayer$, $aPath$);
					$\mathcal{R}$ $\leftarrow$ $L_2[i]$; \\
					$L_1$, $L_2$ $\leftarrow$ [], []; \\
					nextOpID++; \\
				}
			}
		}	        
		
	}					
	%			\Function{reinitTree}{$newRH$, $childLayer$, $aPath$} \textbf{private}
	%			\State \textbf{assert}(currentSubLayer.len == $childLayer.len$);
	%			
	%			\State parentRootHash = $newRH$;
	%			
	%			\For{$\{i = 0; ~i < childLayer.len ; ~\plusplus{i}\}$}
	%			\State currentSubLayer[i] =  $childLayer[i]$;
	%			\EndFor	        
	%			
	%			\State $\mathcal{R}^s$ = reduceMT(currentSubLayer, currentSubLayer.len);
	%			\State checkSubtreeConsistency($\mathcal{R}^s$, $aPath$, parentRootHash);			
	%			\EndFunction										
	\caption{Introduction of a new $\mathcal{R}$ in $\mathbb{S}$}\label{alg:new-parent-tree}
	\vspace{-0.1cm}
\end{algorithm}

\subsection{Depletion of OTPs}\label{sec:depletion-of-otps}
Even with the previous modification, the number of OTPs remains bounded, therefore they may be depleted.
We propose handling of depleted OTPs by a special operation that replaces the
current tree with a new one.
%
To introduce a new tree securely, we propose updating $\mathcal{R}$ value while using the last OTP of the current tree for confirmation.  
%
%Since the validity of a new $\mathcal{R}$ cannot be verified against any paramount field of the smart contract, 
Nevertheless, for this purpose we cannot use $\Pi_O$ consisting of two stages, as $\mathcal{A}$ possessing $SK_{\mathbb{U}}$ could be ``faster'' than the user and might initialize the last operation and thus block all the user's funds.
If we were to allow repeated initialization of this operation, then we would create a race condition issue.
%


To avoid this race condition issue, we propose a protocol $\Pi_{NR}$ that replaces $\mathcal{R}$ during three stages of interaction with the blockchain, which requires two append-only lists $L_1$ and $L_2$ (see \autoref{alg:new-parent-tree}):
%
\begin{compactenum}
	\item $\mathbb{U}$ enters $OTP_{N-1}$ to $\mathbb{C}$. 
	$\mathbb{C}$ sends  $h(OTP_{N-1} ~\|~ \mathcal{R}^{new})$ to $\mathbb{S}$, which appends it to $L_1$.
	
	\item $\mathbb{C}$ sends $\mathcal{R}^{new}$ to $\mathbb{S}$, which appends it to $L_2$.
	
	\item $\mathbb{C}$ passes $OTP_{N-1}$ with $\pi_{N-1}$ to $\mathbb{S}$, where the first matching entries of $L_1$ and $L_2$ are located to perform the introduction of $\mathcal{R}^{new}$.
	%Note that additionally to OTP with its proof that together confirm the authenticity of a new root hash, we provide this function with the cached layer (i.e., $childLayer$) of the first child tree belonging to the new parent tree and with the authentication path (i.e., $aPath$) that serves for the consistency verification of the new child cached layer (and its child root hash) against the new parent root hash.
	%Storing and consistency verification of the child cached layer is performed in the function $reinitParentTree()$ that also updates the parent root hash.
	Finally, the lists are cleared for future updates.
	%
\end{compactenum}

\noindent
Locating the first entries in the lists relies on the append-only feature of lists, hence no $\mathcal{A}$ can make the first valid pair of entries in the lists.
%
Similarly as in $\Pi_{B}$, we propose two variants of $\Pi_{NR}$ intended for secure (i.e., $\Pi_{NR}^\mathcal{S}$) and insecure environment (i.e., $\Pi_{NR}^\mathcal{I}$).
%
In $\Pi_{NR}^\mathcal{I}$ (see Appendix~\ref{appendix:protocols}), $\mathbb{A}$ must compute and display $h(OTP_{N-1} ~\|~ \mathcal{R}^{new})$ and $\mathcal{R}^{new}$ to enable protection against $\mathcal{A}$ that tampers with $\mathbb{C}$. 
Hence, $\mathbb{U}$ can verify the equality of items displayed at $\mathbb{W}$ with the ones displayed at $\mathbb{A}$ during the first and the second stage of $\Pi_{NR}^{\mathcal{I}}$, preventing $\mathcal{A}$ from forging the tree.
%
%(see \autoref{eqn:alpha-beta-final}).\footnote{Note that equation contains further, not yet introduced, optimizations.}
%
%\begin{eqnarray}\label{eqn:hash-chains-depletion}
%	\alpha(i) &=& P - \left\lfloor  \frac{\textcolor{blue}{(i ~\%~ N)} P}{N} \right\rfloor - 1,\\
%	\beta(i) &=&  \textcolor{blue}{\left\lfloor \frac{i}{N} \right\rfloor \frac{N}{P} ~+~}  \left( i ~\%~ \frac{N}{P} \right),
%	%getOTP(i) = h^{P - \lfloor  \textcolor{blue}{(i ~\%~ N)} / \frac{N}{P} \rfloor - 1} \left( F_k \left( \textcolor{blue}{\lfloor i / N \rfloor \frac{N}{P} ~+~}  \left( i ~\%~ \frac{N}{P} \right)  \right) \right), 
%\end{eqnarray}
%where $i$ is the ID of operation.
%Note that we depict a difference between the current formula and \autoref{eqn:hash-chains} by blue color.
%
To adapt this improvement at $\mathbb{C}$, $\mathbb{C}$ needs to store all nodes of the new tree.
Therefore, $\mathbb{U}$ provides $\mathbb{C}$ with all nodes of the new tree, transferred from $\mathbb{A}$ on a microSD card.
%
%
In the case of $\Pi_{NR}^\mathcal{S}$, the nodes of the new tree are transferred by a transcription of $k$ from $\mathbb{A}$ to $\mathbb{C}$ and no values are displayed at $\mathbb{W}$ and $\mathbb{A}$ for $\mathbb{U}$'s verification.
%Therefore, the user provides $\mathbb{C}$ with $k$ again (i.e., protocol $\Pi_{NR}^\mathcal{S}$).
%Alternatively, the new leaves can be transferred by a microSD card, if an insecure environment is considered (i.e., protocol $\Pi_{NR}^\mathcal{I}$).
%Once the leaves are computed, the client replaces its storage with the new leaves and then deletes the OTPs and $k$.
%We refer the reader to Appendix~\ref{appendix:protocols} for a detailed description of both protocols \todo{drop}.


\subsection{Cost \& Security Optimizations }\label{subsec:caching-smart-contract}

\subsubsection{\textbf{Caching in the Smart Contract}}\label{sec:caching-smart-contract}
With a high Merkle tree, the reconstruction of $\mathcal{R}$ from a leaf node may be costly.
Although the number of hash computations stemming from the Merkle tree is logarithmic in the number of leaves, the cost imposed on the blockchain platform may be significant for higher trees.
We propose to reduce this cost by caching an arbitrary tree layer of depth $L$ at $\mathbb{S}$ and do proof verifications against a cached layer.
Hence, every call of \textit{deriveRootHash()} will execute $L$ fewer hash computations in contrast to the version that reconstructs $\mathcal{R}$, while $\mathbb{C}$ will transfer by $L$ fewer elements in the proof. % of a transaction/ containing \textit{confirmOp()} call.

The minimal operational cost can be achieved by directly caching leaves of the tree, which accounts only for hash computations coming from hash chains, not a Merkle tree.
However, storing such a high amount of cached data on the blockchain is
too expensive. 
Therefore, this cost optimization must be viewed as a trade-off between the depth $L$ of the cached layer and the price required for the storage of such a cached layer on the blockchain (see
\autoref{sec:costs-analysis}). % where an optimal $L$ is determined).
%

We depict this modification in the left part of \autoref{fig:overview}, and we show that an optimal caching layer can be further partitioned into caching sublayers of subtrees (introduced later).
%The right part of \autoref{fig:overview} shows how we combine Merkle tree and hash chains.
%
To enable this optimization, the cached layer of the Merkle tree must be stored in the constructor of $\mathbb{S}$. % alongside of $\mathcal{R}$.
%\footnote{Optionally, $\mathcal{R}$ can be passed to the constructor as well, enabling the enforcement of a consistency check of the cached layer.}
%In the constructor, the consistency of the cached layer against $\mathcal{R}$ is necessary to verify with help of function \textit{reduceMT()} from \autoref{alg:MT-reduce-root}. 
From that moment, the cached layer replaces the functionality of $\mathcal{R}$,  reducing the size of proofs.
During the confirmation stage of $\Pi_{O}$, an OTP and its proof are used for the reconstruction of a particular node in the cached layer, instead of $\mathcal{R}$.
Then the reconstructed value is compared with an expected node of the cached layer.
The index of an expected node is computed as 
%
\begin{eqnarray}
 idxInCache(i) &=&	\left\lfloor \left(i ~\%~ \frac{N}{P} \right)  ~/~ 2^{H - L} \right\rfloor, 
\end{eqnarray}
where $i$ is the ID of an operation.

%Then, the index of the confirmed operation $opID$ has to be modified to fit the range covered by an expected node in the cached layer, which is done by clearing $L$ most significant bits of $opID$.
%\feedback{IH: maybe put alg. as it is a contribution?}

\vspace{-0.1cm}
\subsubsection{\textbf{Partitioning to Subtrees}}
The caching of the optimal layer minimizes the operational costs of SmartOTPs, but on the other hand, it requires prepayment for storing the cache on the blockchain.
If the cached layer were to contain a high number of nodes, then the initial deployment cost could be prohibitively high, and moreover, the user might not deplete all the prepaid OTPs.
On top of that, after revealing the first iteration layer of OTPs, the security of our scheme described so far is decreased by $log_2(N/P)$ bits due to the birthday attack (see \autoref{sec:analysis}) on OTPs. % in the same iteration layer. 
Hence, bigger trees suffer from higher security loss than smaller trees. 
%

To overcome the prepayment issue and to mitigate the birthday attack, we propose partitioning an optimal cached layer to smaller groups having the same size, forming sublayers that belong to subtrees (see the left part of \autoref{fig:overview}).
The obtained security loss is $log_2(N_S/P)$, $N_S \ll N$.

%\footnote{Although such an aggregation can be extended to arbitrary number of levels, for demonstration purposes we selected 2 levels only.} 
%
Starting with the deployment of $\mathbb{S}$, the cached sublayer of the first subtree and the ``parent'' root hash (i.e., $\mathcal{R}$) are passed to the constructor; the cached sublayer is stored on the blockchain and its consistency against $\mathcal{R}$ is verified.
%
Then during the operational stage of $\Pi_{O}$, when confirmation of operation is performed, the passed OTP is verified against an expected node in the cached sublayer of the current subtree, saving costs for not doing verification against $\mathcal{R}$ (see \autoref{alg:MT-deriveNodeInCache-hash-chains} in Appendix).

If the last OTP of the current subtree is reached, then no operation other than the introduction of the next subtree can be initialized (see the green dashed arrow in \autoref{fig:overview}).
%
We propose a protocol $\Pi_{ST}$ for the introduction of the next subtree (see Appendix~\ref{appendix:protocols} for the detailed description).
Namely, $\mathbb{C}$ introduces the next subtree in a single step by calling a function \textit{nextSubtree()} of $\mathbb{S}$ with the arguments containing:
(1) the last OTP of the current subtree $OTP_{(N_S - 1) + \delta N_S}, ~\delta \in \{1, ~\ldots,~ N/N_S - 1\}$, 
(2) its proof $\pi_{otp}$, 
(3) the cached sublayer of the next subtree, and 
(4) the proof $\pi_{sr}$  of the next subtree's root; all items but OTP are computed by $\mathbb{C}$. % from its storage.
%
% This operation is performed in a single step, requiring user's signature as well as the last OTP belonging to the current subtree.
%
\begin{algorithm}[t]
	\caption{Introduction of the next subtree at $\mathbb{S}$}\label{alg:alg-next-child-tree}	
	
	\footnotesize
	
	\SetKwProg{func}{function}{}{}
	
	currentSubLayer[]; \Comment{Adjusted in the constructor} \\
%	parentRootHash; \Comment{Adjusted in the constructor} 
	\smallskip		
	
	\func{$nextSubtree$(nextSubLayer, otp, $\pi_{otp}$, $\pi_{sr}$) \textbf{public}}{ 
%		\textbf{assert} \textit{sender} = owner;\\
		\textbf{assert} nextOpID $\%~N$ $\neq N - 1$; \Comment{Not the last op. of parent}\\
		\textbf{assert} nextOpID $\%~N_S$ $ = N_S - 1 $; \Comment{The last op. of subtree}\\
		\textbf{assert} currentSubLayer.len = nextSubLayer.len;\\

%		verifyOTP(otp, $\pi_{otp}$, nextOpID);\\
		\textbf{assert} deriveRootHash(otp,  $\pi_{otp}$, nextOpID) = $\mathcal{R}$;\\				
		
		currentSubLayer $\leftarrow$  nextSubLayer;\\
		
		$\mathcal{R}^s$ $\leftarrow$ reduceMT(currentSubLayer, currentSubLayer.len);\\
		\textbf{assert} subtreeConsistency($\mathcal{R}^s$, $\pi_{sr}$, $\mathcal{R}$);\\
		nextOpID++;  \Comment{Accounts for this introduction of a subtree}\\			
	}			
	%	\vspace{-0.5cm}						
\end{algorithm}
%
The pseudo-code of the next subtree  introduction at $\mathbb{S}$ is shown in \autoref{alg:alg-next-child-tree}. 
The current subtree's cached sublayer is replaced by the new one, which is verified by the function $subtreeConsistency()$
%\footnote{We do not provide pseudo-code of this function, as it	is similar to the function $verifyOTP()$ from \autoref{alg:wallet-overview}.} 
against $\mathcal{R}$ with the use of the passed proof 
$\pi_{sr}$ of the new subtree's root hash $\mathcal{R}^s$.
%\footnote{Although the term ``authentication path'' can also be denoted as a proof, we have decided to use this term here to distinguish between a proof of an OTP and a proof of the next subtree's cached layer.} 
Note that introducing a new subtree invalidates all initialized yet to be confirmed operations of the previous subtree.
%
%We remark that when the next subtree's cache is adjusted, the ``new'' OTPs are used in the same way as in the case of the previous subtree.
%

At $\mathbb{A}$, this improvement requires accommodating the iteration over layers of hash chains in shorter periods.
Hence, $\mathbb{A}$ provides OTPs by \autoref{eqn:hash-chains} with the following expressions:
%
\begin{eqnarray}\label{eqn:alpha-beta-final}
\begin{split}
	\alpha(i) &=& P - \left\lfloor   \frac{(i ~\%~ N_S) P}{N_S} \right\rfloor - 1,\\
	\beta(i) &=&  \left\lfloor \frac{i}{N_S} \right\rfloor \frac{N_S}{P} +  \left( i ~\%~ \frac{N_S}{P} \right),
%
%getOTP(i) = h^{P - \lfloor  (i ~\%~ N_S) / \frac{N_S}{P} \rfloor - 1} \left( F_k \left( \lfloor i / N_S \rfloor \frac{N_S}{P} +  \left( i ~\%~ \frac{N_S}{P} \right)  \right) \right), 
\end{split}
\end{eqnarray}
where $i$ is an operation ID and $N_S$ is the number of OTPs provided by a single subtree.
%Note that we depict a difference between the current formula and \autoref{eqn:hash-chains-depletion} by blue color.
%
We remark, that due to this optimization, the update of a new parent root $\mathcal{R}$ as well as the constructor of $\mathbb{S}$ requires, additionally to \autoref{alg:new-parent-tree} and \autoref{alg:wallet-overview}, the introduction of a cached sublayer of the first subtree (omitted here for simplicity).

%Moreover, to protect this protocol from tampering with the client, $\mathbb{A}$ displays a message confirming that the next subtree is being introduced, and $\mathbb{U}$ transfer OTP only when he sees this message. % This is nice, but is is out-of-the scope, since it assumes a combinattion of 2 attacker model (tampering with the client +possessing SK_U)




==> sec/discussion.tex <==
%Although the Merkle scheme has interesting security and usability properties, its main drawback is that the number of OTPs is limited.
%However, based on our analysis of Ethereum blockchain we expect that a size of 1024 is enough for a wallet of a regular user.
%Considering the richest 5000 \textit{regular addresses} of Ethereum,\footnote{\url{https://etherscan.io/accounts/}, as of 27th of June 2018.} we found out that the median of transfer count is equal to $10$, while $96.02\%$ and $90.21\%$ of addresses have fewer than 1024 and 128 transfers executed, respectively.
%Analyzing the richest 5000 \textit{smart contract addresses} of Ethereum, we found out that the median of transfer count is equal to $68$, while $85.95\%$ and	 $67.22\%$ smart contracts have fewer than 1024 and 128 transfers executed, respectively.

%For clarity, we assumed only a single Merkle tree associated with the authenticator, which has a negative impact on the usability of our framework when OTPs are depleted, causing that a user has to change an address of his wallet.
%However, the authenticator can be implemented in a similar way as hierarchical deterministic wallets, but in contrast requiring a recovery phrase $p$ to generate a sequence of authenticator's seeds $k_i, ~|~i \in \mathbb{N}_0$ by $F_p()$.
%Hence, $p$ would be transferred from the authenticator to the client at the bootstrapping. 
%Then the client would generate and store caches linked to the first e.g., $2^{10}$ Merkle trees, which in the case of $S=16B$ and $N=1024$ would mean storing 16MB of data at the client while providing $2^{20}$ OTPs.  
%Thus, our solution would become more usable even for hosted wallets and cryptocurrency exchanges -- considering the previous list of the richest 5000 smart contract addresses,  there is $99.33\%$ of smart contract address with fewer transfers than $2^{20}$, while in the case of regular addresses it is $99.81\%$.


%\paragraph{\textbf{Passwords}}
%For simplicity, in the description of our approach we abstracted from password protection at $\mathbb{A}$ and $\mathbb{W}$.
%However, to achieve $(2 + 1/1)$-factor authentication (see \autoref{sec:classification}), it is necessary to set them up.
%This authentication scheme represents signatures made by $SK_{\mathbb{U}}$ and OTPs from $\mathbb{A}$ + a password to access $\mathbb{W}$ and a password to access $\mathbb{A}$.



\paragraph{\textbf{Vulnerability in HW Wallets}}
We found out that two used hardware wallets do not display all data of transactions being signed: Trezor One displays first 24B of data and Trezor T displays 35B.
With regard to Ethereum transactions, this means that used wallets display only the first 8B and 19B of data representing the parameters of a contract call. 
Hence, $\mathcal{A}$ that tampers with $\mathbb{C}$ might purposely preserve user expected values in the displayed data while forging data that are not displayed. 
We reported this vulnerability to the vendor, and as a mitigation, we put the most critical parameter (i.e., address) of all concerning functions at the first displayed position.


\paragraph{\textbf{Usability}}
Our approach inherits the common usability characteristics of 2FA schemes, such as an extra device to carry,\footnote{Assuming that the user already has a hardware wallet (the first factor).} effort for securely storing the recovery phrase $k$, effort for recalling/entering passwords, and effort for a transfer of OTPs, which can be made by scanning a QR code or transcription of mnemonic words. % if $\mathbb{C}$ is not equipped with a camera.
%which, according to Dhakal et al.~\cite{Dhakal-typing-study}, takes 14s on average.
Note that these usability implications are almost the same as in the case of existing smart contract wallets with 2FA~\cite{ConsenSys-gnosis,TrezorMultisig2of3}.
%Alternatively, the user might have only a single hardware wallet (instead of two), while $\mathbb{A}$ can be realized as an App on a smartphone, which most of the ordinary users already possess.\footnote{Note that several smartphone vendors provide a dedicated sandboxed environment with encrypted storage for running of security-critical Apps.}
%
In addition to the previous, SmartOTPs requires $\mathbb{U}$ to introduce a new subtree/parent tree once in a while. 
Nevertheless, we envision this effort to be related only to large businesses rather than regular users; 
considering the example from \autoref{sec:fiat-money}, $\mathbb{U}$ has to introduce the next subtree after using $\sim32K$ OTPs, while $\sim33.5M$ OTPs are available to use before re-initialization of the parent tree.
%
Next, we note that entering $opID$ into $\mathbb{A}$ might be seen as a usability limitation, especially when $N$ is large.
However, $opID$ can be reset after each iteration layer of the current subtree, thus fitting a small range (i.e., $\langle1,\frac{N_S}{P}\rangle$). % which is convenient for $\mathbb{U}$.

To compare SmartOTPs with Gnosis Wallet~\cite{ConsenSys-gnosis}, we counted the number of elementary actions (i.e., clicks, button presses, inputs of form fields, QR code scanning) required to make a transfer of funds. 
In the result, SmartOTPs required $33$ actions while Gnosis wallet required $39$ actions. 
%note that a high number of actions were made in Metamask that provisioned a connection to hardware wallet(s). 



\paragraph{\textbf{Costs}}
With consumption of up to $\sim150k$ gas units per operation, our approach is comparable to equivalent 2FA solutions using smart contracts: Gnosis Wallet~\cite{ConsenSys-gnosis} requires $\sim275k$ gas units\footnote{\href{https://etherscan.io/tx/0xdb6e9389530a5fa51a43593ac57c3343400fa39ced624d94e266cca4d2b5c09c}{https://etherscan.io/tx/0xdb6e938...} and \href{https://etherscan.io/tx/0x328a7cc75788e0b02a4aa6c7b0ade997c70b3f92522c1ef72f82355bfa2a9455}{https://etherscan.io/tx/0x328a7cc...}} and TrezorMultisig2of3~\cite{TrezorMultisig2of3} requires $\sim95k$ gas units\footnote{\href{https://etherscan.io/tx/0xfc7bbddd8ae58190b5543ed7122e9b52bd67412ffd6b7024e1221d8c80e1229c}{https://etherscan.io/tx/0xfc7bbdd...} (2 signatures in a single transaction).} per operation.

%
%\textcolor{red}{On the other hand, in contrast to our approach, we demonstrated that common 2FA schemes do not meet the usability requirements in an air-gapped setting or require a shared secret (see \autoref{sec:design-space}).}

%\paragraph{\textbf{Sustainability of Blockchain}}
%A space required for storing a cached layer of the Merkle tree affects the size of a blockchain.
%On the other hand, a natural incentive of the user is to maximize a saving by caching, regardless of the sustainability of a blockchain.

\paragraph{\textbf{Lost Secrets}}
When $\mathbb{U}$ loses access to $\mathbb{A}$, he can initialize a new instance of $\mathbb{A}$ from the backup of seed $k$.
Moreover, if $\mathbb{U}$ losses access to $\mathbb{A}$ and $\mathbb{W}$ at the same time, he can still recover the funds with the last resort functionality that we implemented (see \autoref{sec:implementation}).


\paragraph{\textbf{State at the Client}}
The only state $\mathbb{C}$ has to store is the cache of hashes of OTPs from the first iteration layer. 
This might be seen as a limitation when $\mathbb{U}$ changes a client device. 
However, the state can be recovered anytime from the seed $k$ or transferred by microSD card from $\mathbb{A}$ to $\mathbb{C}$ (see \autoref{sec:bootstraping-sec} and \autoref{sec:bootstraping-insec}).

\paragraph{\textbf{Transaction Size}}
Although the base version of SmartOTPs might slightly bloat the transaction due to $H$ items of the proof, this is improved with the caching at $\mathbb{S}$, which reduces the number of items in the proof to $H$ - $L$.
For example, in the case of $H=10$ and optimal caching (see \autoref{sec:costs-MK}) where $L=7$, only three items of the proof are required.
In this case, SmartOTPs consume ~68B of transaction data (assuming 4B for operation ID), which is similar to asymmetric cryptography used in most of the blockchains.

%\paragraph{\textbf{General Purpose Applicability}}
%In this work, we focused on smart contract wallets.
%However, we remark that the protocols of our scheme can be utilized in any smart contract based application for the purpose of 2FA.

%\paragraph{\textbf{Sustainability}}
%\todo{Big cache at blockchain}
	
%Next, our approach can be extended in order to eliminate evil maid attacker model targeting the authenticator device.
%In this attack, a user's device is stolen and replaced by a foisted one with an intention to extract user's access/encryption password configured on an original device, while assuming an interception of communication between the client and the smart contract. 
%%
%Therefore, we enable a user to configure secondary password at the authenticator, which is used for symmetric encryption/decryption of his pre-specified phrase~\cite{BitLox}. 
%If the pre-specified phrase is displayed after entering this password, a user knows that his device was not foisted.

%	These are well-known security enhancements of authentication schemes~\cite{Armory-SW-Wallet, mycelium-wallet}.
	
%    \psz{this discussion is very short. I'd drop it, just moving the forks part to security analysis} 





==> sec/implementation.tex <==


We have selected the Ethereum platform and the Solidity language for the implementation of $\mathbb{S}$,
HTML/JS for DAPP of $\mathbb{C}$, Java for smartphone App of $\mathbb{A}$,
%\footnote{Note that the authenticator App does not require any permissions.}
 and Trezor T\&One~\cite{trezor-hw-wallet} for $\mathbb{W}$.
%We highlight that we instantiated $\mathbb{W}$ by Metamask only for a proof-of-concept purpose, since Metamask is a password-derived software wallet, and thus it does not provide a resilience against adversary that tampers with the client (see \autoref{sec:analysis}).
%Although our approach provides 2-factor authentication, we demonstrate its proof-of-concept in the setting of 2-step authentication, since the authenticator is an application and not a dedicated hardware device (see \autoref{sec:pre}).
%, thus implementing 2SA, not 2FA.
% The later two components serve just for the proof-of-concept purposes, and therefore their provide only minimal functionality.
%
%The smart contract, the private key wallet, and the client are cryptocurrency-specific components, while the authenticator is cryptocurrency-agnostic and thus can be directly reused in any other cryptocurrencies with similar capabilities.
% We emphasize that the major part of the client can be reused as it is in other smart contract languages. 
% The only required modification is to replace the adapter for calling smart contract transactions.
%
We selected $S=128$ bits, which has practical advantages for an air-gapped $\mathbb{A}$, producing OTPs that are 12 mnemonic words long or a QR code v1 (with a capacity of 17B).
%\footnote{Considering a dictionary size of 2048 words~\cite{bipMnemonic}.} 
%and at the same time, providing a sufficient security level for most use cases. 
%
Next, we used SHA-3 with truncated output to 128 bits as $h(.)$. % as well as an instantiation of $F_k(.)$. % $\equiv h(k ~||~.)$.
%by AES in the counter mode.
%SHA-3 hash function has the output of 256 bits, which is shrank to 128 bits in the case of (i.e., 16B).
%
We selected the size of $k$ equal to 128 bits, fitting 12 mnemonic words $\simeq$ 1 QR code v1.
%

So far, we have considered only the crypto-token transfer operation.
However, our proposed protocol enables us to extend the set of operations.
%
For demonstration purposes, we extended the operation set by supporting daily limits and last resort information (see Appendix \ref{sec:functionality-extension}). % which also contribute to the increased security of SmartOTPs.
%
We also tested our contracts by static/dynamic analysis tools Mythril~\cite{mythrill}, Slither~\cite{slither}, and ContractGuard~\cite{ContractGuard-fuzzer}; none of them detected any vulnerabilities. % and ContractGuard ranked our code as excellent.
%
In addition, we made a hardware implementation of $\mathbb{A}$ using Node\-MCU~\cite{node-mcu} equipped with ESP8266 (see Appendix~\ref{appendix:NodeMcu-schema}).
The source code of our implementation and videos are available at~\url{https://www.dropbox.com/sh/gmcz8zt12j7omsf/AADR4LHDOhSlwANnI707gkMda?dl=0}. % and contains $\sim6~KLOC$. % (see \autoref{tab:loc} in Appendix).	


%\subsection{Evaluation of the Functionality}		
%\psz{why here?}
%To evaluate the functionalities of our proposed solution and its extensions, we implemented several unit test suites in the Truffle framework\psz{discuss}. 
%The additional purpose of these unit tests is to measure the price of each transaction call for further analysis.

%
%\feedback{Comment out after this?}
%%
%The unit tests evaluate normal run of the initialization and the confirmation of transfer operations, while also expected behavior during the \textit{confirmOp()} with wrong / previously used confirmation material is tested.
%Testing the adjustment and exceeding of daily limits is covered by dedicated test suite. 
%%We also perform testing of accumulated daily expenses with regards to the time.
%Then we aim at testing of the last resort functionality where various adjustments of these values and times shifts are performed.
%%
%As the number of confirmation materials in the Merkle tree scheme is limited, we test the correct functionality of the buffer of pending operations, its clearing mechanism, and a depletion of confirmation materials.
%






==> sec/intro.tex <==
% this one? - https://en.wikipedia.org/wiki/BitGo#Bitfinex_Hack

%\bookmark{Motivation + incidents}
The success of cryptocurrencies has surpassed all expectations resulting in various open and decentralized platforms that allow users to conduct monetary transfers, write smart contracts, and participate in predictive markets.  
%Cryptocurrencies promise to revolutionize many fields and businesses.
Cryptocurrencies introduce their own crypto-tokens, which can be transferred in transactions authenticated by private keys that belong to crypto-token owners.
These private keys are managed by a wallet software that gives users an interface to interact with the cryptocurrency.
There are many cases of stolen keys that were secured by various means~\cite{2016-brainwallets,courtois2016speed,CHHMPRSS18,binance-hack-2019}.
%
Such cases have brought the attention of the research community to the security issues related to key management in cryptocurrencies~\cite{eskandari2018first,goldfeder2015securing,2015-Bitcoin-SOK}.
According to the previous work~\cite{eskandari2018first,2015-Bitcoin-SOK}, there are a few categories of key management approaches. % in Bitcoin also applicable to other cryptocurrencies.

% Local wallets
In pass\-word-protected wallets, private keys are encrypted with selected passwords.
Unfortunately, users often choose weak passwords that can be brute-forced if stolen by malware~\cite{2015-CCSM-SecureWorks}; optionally, such malware may use a keylogger for capturing a passphrase~\cite{2015-Bitcoin-SOK,2017-keylogger-bc-malware}.
%
Another similar option is to use password-derived wallets that generate keys based on the provided password.
However, they also suffer from the possibility of weak passwords~\cite{courtois2016speed}. 
%Moreover, the recent research also made advancements in the speedup of brute force attacks against brain wallets, which enabled to crack more complex passwords~\cite{courtois2016speed}.
%
Hardware wallets are a category that promises the provision of better security by introducing devices that enable only the signing of transactions, without revealing the private keys stored on the device.
However, these wallets do not provide protection from an attacker with full access to the device~\cite{kraken-trezor-hack,kraken-keepkey-hack,donjon-ellipal-hack}, and more importantly, wallets that do not have a secure channel for informing the user about the details of a transaction being signed (e.g.,~\cite{ledger-nano}) may be exploited by malware targeting IPC mechanisms~\cite{bui2018man}.
%

% Hosted wallets & exachnge services
A popular option for storing private keys is to deposit them into  server-side hosted (i.e., custodial) wallets and currency-exchange services~\cite{CoinbaseWallet,binance-exchange,poloniex-exchange,kraken-exchange,luno-wallet,paxful-wallet}.
In contrast to the previous categories, server-side wallets imply trust in a provider, which is a potential risk of this category.
%
Due to many cases of compromising server-side wallets~\cite{2018-coindesk-bithumb,2014-Mt-Gox,2016-Bitfinex-hack,moore2013beware,binance-hack-2019} or fraudulent currency-exchange operators~\cite{vasek2015there}, client-side hosted wallets have started to proliferate.
In such wallets, the main functionality, including the storage of private keys, has moved to the user side~\cite{mycelium-wallet,CarbonWallet,CitoWiseWallet,coinomi-wallet,InfinitoWallet};
hence, trust in the provider is reduced but the users still depend on the provider's infrastructure.

%Alternatively, this category contains wallets that store only encrypted versions of keys by a third party  \cite{BTC-com-wallet,BlockchainInfoWallet}.

To increase security of former wallet categories, multi-factor authentication (MFA) is often used, which enables spending crypto-tokens only  when a number of secrets are used together.
However, we emphasize that different security implications stem from the multi-factor authentication made \textit{against a centralized party} (e.g., using Google Authenticator) and \textit{against the blockchain} itself.
In the former, the authentication factor is only as secure as the centralized party, while the latter provides stronger security that depends on the assumption of an honest majority of decentralized consensus nodes  (i.e., miners) and security of cryptographic primitives used. 
%since validations of all factors are executed by all miners respecting rules of the consensus protocol.
%
Wallets from a split control category~\cite{eskandari2018first} provide MFA against the blockchain.
This can be achieved by threshold cryptography wallets~\cite{goldfeder2015securing,mycelium-entropy}, multi-signature wallets~\cite{Armory-SW-Wallet,Electrum-SW-Wallet,TrustedCoin-cosign,copay-wallet}, and state-aware smart-contract wallets~\cite{TrezorMultisig2of3,parity-wallet,ConsenSys-gnosis}.
% that are based on Turing-complete smart contract blockchains.
The last class of wallets is of our concern, as spending rules and security features can be encoded in a smart contract. % hence, it can be adjusted almost arbitrarily to the user's needs.

Although there are several smart-contract wallets using MFA against the blockchain~\cite{TrezorMultisig2of3,ConsenSys-gnosis}, to the best of our knowledge, none of them provide an air-gapped authentication in the form of short OTPs similar to Google Authenticator. % which is the focus of our work.

\paragraph{\textbf{Proposed Approach}}
In this paper, we propose SmartOTPs, a framework for smart-contract  cryptocurrency wallets,
%\footnote{Further interchangeably denoted with term smart contract.}
%...that encodes and enforces the user's policy regarding spending rules. 
%
%Unlike traditional one-size-fits-all solutions, smart contract wallets allow users to customize their wallets to a high extent, similarly to the way they customize their bank accounts or credit cards.
%
which provides 2FA against data stored on the blockchain.
The first factor is represented by the user's private key and the second factor by OTPs.
% and it is accomplished by: 1) a client, 2) a private key hardware wallet, 3) a smart-contract, and 4) an air-gapped authenticator; forming the same number of components as present in other equivalent solutions~\cite{TrezorMultisig2of3,ConsenSys-gnosis}.
To produce OTPs, the authenticator device of SmartOTPs utilizes hash-based cryptographic constructs, namely a pseudo-random function, a Merkle tree, and hash chains.
We propose a novel combination of these elements that minimizes the amount of data transferred from the authenticator, which enables us to implement the authenticator in a fully air-gapped setting, not requiring any USB or another connection. 
%In addition to that, our construction protects users' crypto-tokens from advances in quantum computing, which would make deployed asymmetric algorithms potentially insecure.
%
SmartOTPs belongs to the category of state-aware smart contract wallets, and it provides protection against the attacker that possesses the user's private key \textit{or} the user's authenticator \textit{or} the attacker that tampers with the client. % (each assumed exclusively). 
%SmartOTPs framework provides a cheap extension of security level of hardware wallets by adding 2nd factor.

% Man-in-the-Machine attacker (MitMa)~\cite{bui2018man} if used with particular type of hardware wallets, and resilience against quantum computing. 
% and a few useful customizable security features.
% and in contrast to the existing solutions~\cite{ConsenSys-gnosis,TrezorMultisig2of3}, 
%
%Our solution primarily provides 2-step authentication that defends against stolen private keys of clients. 
%, but we additionally consider attacker who has an access to authenticator device.
%Moreover, when combined with a hardware wallet, SmartOTPs provide resilience against tampering with the client.

%\paragraph*{\textbf{Attacker Models}}
%\psz{It is definitely not a good place for that. I suggest to drop it (it is in the background section anyway).}
%Our proposed approach is resistant against several attacker models.
%In the first attacker model, we assume that user's private key associated with his cryptocurrency account has been stolen by an attacker.
%The second attacker model is an extension of the first attacker model.
%Thus, we assume an attacker who already possesses the user's private key, while he can moreover intercept and modify the user's communication with the blockchain of a cryptocurrency.
%%On the other hand, we do not assume that an attacker can tamper the client or extract secret material from authenticator.
%Additionally to these attacker models, we propose countermeasures for the attacker models that represents: tampering with the client, evil maid attacker, and scam version of the authenticator.


\paragraph{\textbf{Contributions}}
Our main contributions are as follows:
%In this work we make the following contributions.
\begin{compactitem}
%	We also categorize existing cryptocurrency wallet solutions according to this notion.

    \item We show that standard 2FA methods against the blockchain do not meet either the security or usability requirements for an air-gapped setting (see \autoref{sec:design-space}).
    % and are prone to quantum computing attacks.

    \item We propose SmartOTPs, a smart-contract wallet framework that provides 2FA against the blockchain while using short OTPs serving as the second factor (see \autoref{sec:overview}).     
    OTPs are managed in a novel way,  enabling us to make an authenticator device fully air-gapped. 
%	We achieve this by delegating a Merkle proof construction at the client that stores non-confidential data of the Merkle tree. 
	
	\item To increase the number of OTPs, we resolve the time-space trade-off at the client by combining hash chains with Merkle trees in a novel way (see \autoref{sec:increasingNoOfOTPs}).
   
	\item We implement and evaluate our approach (including hardware version of the authenticator), and we provide the source code of our solution (see \autoref{sec:implementation}). 
%	The provided smart contract is self-contained, but its operation set can be extended by the community.
	
%	\item We introduce and formalize the notion of $k$-factor authentication against the blockchain and $k$-factor authentication against the authentication factors (see \autoref{sec:related}).
%	Using these notions, we propose a classification of authentication schemes, and we apply it to related work.
	
\end{compactitem}



% \paragraph*{\bookmark{Paper Organization (Optional)}}



==> sec/overview.tex <==
% For a generic cryptocurrency described in \autoref{sec:pre}, we propose a 2-step authentication solution that is, by design, resistant against an attacker who stole the user's private key and, who moreover can intercept and modify user's transmitted data to the blockchain -- attacker models A) and B).
% %
% Additionally, our proposed solution is made resistant against an attacker who tampers with the client, then against scam of the authenticator, and also against an evil maid attack with the authenticator device -- attacker models C), D), and E).
%\footnote{This is achieved by a redundancy that consider two clients running on dedicated devices each, where one instance is watch-only.}
%

For a cryptocurrency described in \autoref{sec:pre}, we propose SmartOTPs, a 2FA against the blockchain, which consists of: (1) a client $\mathbb{C}$, (2) a private key hardware wallet $\mathbb{W}$ equipped with a display, (3) a smart-contract $\mathbb{S}$, and (4) an air-gapped authenticator $\mathbb{A}$ that might be implemented as an embedded device with limited resources.
First, we explain the key idea of our approach, which enables us to construct $\mathbb{A}$ as a fully air-gapped device.
Then, we present the base version of SmartOTPs, and finally, we describe modifications. % that improve the efficiency and practicality of our approach. 



\subsection{Design of an Air-Gapped Authenticator}
In our approach, OTPs are generated by a pseudo-random function $F_k(.)$ and then aggregated by a Merkle tree, providing a single value, the root hash ($\mathcal{R}$).
$\mathcal{R}$ is stored at $\mathbb{S}$ and serves as a PK for OTPs.
%
Assuming the two stage protocol $\Pi_O^{<G>}$ (further denoted as $\Pi_O$), the user $\mathbb{U}$ might confirm the initiated operation $O_{opID}$ by a corresponding $OTP_{opID}$ (provided by $\mathbb{A}$) in the second stage of $\Pi_O$, whereby $\mathbb{S}$ verifies the correctness of $OTP_{opID}$ with use of $\mathcal{R}$.
A challenge of such an approach is the size of an OTP. 
%As we already mentioned in \autoref{sec:design-space}, OTPs in general do not provide non-repudiation of the messages in which they are contained.
%To overcome this limitation, we instantiate the two-stage protocol $\Pi_O^{<G>}$, further denoted as $\Pi_O$.


%In contrast to digital signatures, $\mathcal{R}$ serves only for proving the non-repudiation of a particular OTP, not an arbitrary message.
%To overcome this limitation, we propose a two-stage protocol $\Pi_{O}$, in which, an operation $O$ is first submitted to the blockchain where it obtains an identifier $opID$. 
%Then, in the second stage, $O_{opID}$ is executed upon authentication by $OTP_{opID}$ that is unambiguously associated with the identifier of this operation.


\subsubsection{\textbf{From Straw-Man to the Base Version}}
Using the straw-man version, a 2FA requires $\mathbb{A}$ to provide an OTP and its proof.
However, in such a straw-man version, the user $\mathbb{U}$ has to transfer $\frac{(S + S \times H)}{8}$ bytes from $\mathbb{A}$ each time he confirms an operation, where $S$ represents the bit-length of an OTP as well as the output of $h(.)$, and $H$ represents the height of a Merkle tree with $N$ leaves; hence $H = log_2(N$).
%
For example, if $S = 256$ and $H = 10$, then $\mathbb{U}$ would have to transfer 352B each time he confirms an operation, which has very low usability in an air-gapped setting utilizing transcription of mnemonic words~\cite{bipMnemonic} (i.e., 264 words) or scanning of several QR codes (e.g., 21 QR codes v1) displayed on an embedded device with a small display.
Even further reduction of $S$ to 128 bits would not help to resolve this issue, as the amount of user transferred data would be equal to 176B $\simeq$ 132 mnemonic words $\simeq$ 11 QR codes v1.

We make the observation that it is possible to decouple providing OTPs from providing their proofs.
The only data that need to be kept secret are OTPs, while any node of a Merkle tree may potentially be disclosed -- no OTP can be derived from these nodes.
%\footnote{Although compromising all leaf nodes might slightly simplify a brute-force attack by the birthday paradox (see \autoref{sec:analysis}).}
%\footnote{It is unfeasible to derive OTPs from these nodes, thus a compromised client cannot authenticate any transactions without the authenticator.}
Therefore, we propose providing OTPs by $\mathbb{A}$, while their proofs can be constructed at $\mathbb{C}$ from stored hashes of OTPs. % (or from stored all nodes in optimized version).
This modification enables us to fetch the nodes of the proof from the storage of $\mathbb{C}$, while $\mathbb{U}$ has to transfer only the OTP itself from $\mathbb{A}$ when confirming an operation (i.e, $S = 128 \simeq 12$ mnemonic words by default).



\subsection{Base Version}\label{sec:base-version}
%(e.g., an HTML + JS application)
% (e.g., an air-gapped device or a smartphone application). 
% At the beginning, our approach has to be bootstrapped.
% After the components are initialized, they can be used to run a two-stage
% protocol for authenticating of operations.
% In the following we describe these actions in detail.
%\todo{For clarity we first talk about high level description of our approach.}
%
% The two-stage protocol relies on a functionality of smart contracts and consists of initialization and confirmation stages.
% Hence, all operations with the proposed wallet have to be performed through the predefined functions of the wallet's smart contract.
% %
%
%Also, the smart contract has to be constructed with the knowledge of the public key that is unambiguously associated with the user's authenticator (e.g., $\mathcal{R}$ of Merkle tree or public key of the asymmetric cryptography).
%This binds the user's authenticator with the smart-contract wallet instance, and therefore it enables to verify whether an OTP was produced by the user's authenticator.
%

\begin{algorithm}[t]	
	\caption{Smart contract $\mathbb{S}$ with 2FA}\label{alg:wallet-overview}
	\footnotesize 
	
	\SetKwProg{func}{function}{}{}
	
	$\triangleright$ \textsc{Variables and functions of environment:} \\
	\hspace{1em} \textit{tx}: a current transaction processed by $\mathbb{S}$,\\
	\hspace{1em} \textit{balance}: the current balance of a contract, \\
	\hspace{1em} \textit{transfer(r, v)}: transfer \textit{v} crypto-tokens from a smart contract to \textit{r},\\
	%		\hspace{1em} \textit{revert(m)}: revert an effect of transaction, yielding message \textit{m},\\
	
	\smallskip
	$\triangleright$ \textsc{Declaration of types:}\\
	%		\hspace{1em} \textbf{enum} OpType \{ TRANSFER \}  \\
	\hspace{1em} \textbf{Operation} \{ addr, param, pending, type $\in \{ \text{TRANSFER}, \ldots\}$ \} \\
	
	\smallskip
	$\triangleright$ \textsc{Declaration of functions:}
	
	\func{$constructor$(root, pk) \textbf{public} }{
		operations $\leftarrow$ []; \Comment{An append-only list} \\ 
		$PK_\mathbb{U}$ $\leftarrow$ \textit{pk},
		$~$$\mathcal{R}$ $\leftarrow$ root, 
		$~$nextOpID $\leftarrow$ 0; \\
		%		\Comment{ID of the next operation (opID)}  \\
		\textbf{return} $\mathbb{S}^{ID};$ \Comment{Computed by a blockchain platform.} \\
	}
	
	
	\func{$initOp$(a, p, type) \textbf{public} }{
		\textbf{assert} $\Sigma.verify(tx.\sigma, PK_\mathbb{U})$; \Comment{1st factor of 2FA} \\						
		opID $\leftarrow$ nextOpID$\texttt{++}$; \\
		operations[opID] $\leftarrow$ \textbf{new} Operation(a, p, \textbf{true}, type); \\
		%			nextOpID$\texttt{++}$; \\
	}
	
	\func{$confirmOp$(otp, $\pi$, opID) \textbf{public} } { 
		\textbf{assert}  operations[opID].pending; \\
		verifyOTP(otp, $\pi$, opID); \Comment{2nd factor of 2FA} \\									
		execOp(operations[opID]); \\
		operations[opID].pending $\leftarrow$ \textbf{false}; \\
	}
	
	\func{$verifyOTP$(otp, $\pi_{opID}$, opID) \textbf{private} } {
		\textbf{assert} deriveRootHash(otp, $\pi_{opID}$, opID) = $\mathcal{R}$; \\
	}
	
	\func{$execOp$(oper) \textbf{private} }{
		\If{TRANSFER = oper.type}{
			\textbf{assert} oper.param  $\leq$ \textit{balance}; \\
			\textit{transfer}(oper.addr, oper.param); \\
			
		} 
		%		\Else {
		%				\textit{revert}(``Unknown type of requested operation.''); \\
		%			}					
	}						
%	\vspace{-0.1cm}
\end{algorithm}

\subsubsection{\textbf{Secure Bootstrapping}}\label{sec:bootstraping-sec}
As common in other schemes and protocols, by default, we assume a secure environment for bootstrapping protocol $\Pi_{B}^\mathcal{S}$ (see \autoref{fig:smart-contract-deploy} and Appendix~\ref{appendix:protocols}). 
First, $\mathbb{A}$ generates a secret seed $k$, which  is stored as a recovery phrase by $\mathbb{U}$.
$\mathbb{W}$ generates a key-pair $SK_\mathbb{U}, PK_\mathbb{U} \leftarrow \Sigma.KeyGen()$.
Next, $\mathbb{U}$ transfers $k$ from $\mathbb{A}$ to $\mathbb{C}$ in an air-gapped manner (i.e., transcribing a few mnemonic words or scanning a QR code). 
Then, $\mathbb{C}$ generates OTPs by computing $F_k(i)~|~i \in \{0, 1, \ldots, N-1\}$, where $N$ is the number of leaves (equal to the number of OTPs in the base version).
Next, $\mathbb{C}$ computes and stores the leaves of the tree -- i.e., the hashes of the OTPs (i.e., $hOTPs$), which do not contain any confidential data.\footnote{To improve performance during provisioning of proofs, $\mathbb{C}$ might additionally store non-leaf nodes, increasing the requirement on $\mathbb{C}$'s storage 2x.}
After this step, $k$ and the OTPs are deleted from $\mathbb{C}$, and $\mathbb{C}$ computes $\mathcal{R}$ from the stored hashes of the OTPs.
%
Then, $\mathbb{C}$ creates a transaction containing constructor of $\mathbb{S}$ (see \autoref{alg:wallet-overview}) with $\mathcal{R}$ as the argument and passes it to $\mathbb{W}$ for appending $PK_\mathbb{U}$.
%\footnote{No signature is appended by $\mathbb{W}$ since a secure environment is assumed.}
% which is confirmed by $\mathbb{U}$.
%During a confirmation of the transaction containing a constructor, $\mathbb{U}$ verifies equality of $\mathcal{R}$ displayed by $\mathbb{W}$ and $\mathbb{A}$.
%This step additionally provides a protection against the attacker that tampers with $\mathbb{C}$ and can intercept $k$ but cannot spoof it. %, which in the worst case may degrade our scheme to one factor.
%
Finally, $\mathbb{C}$ sends the transaction with the constructor to the blockchain where the deployment of $\mathbb{S}$ is made.\footnote{$\mathbb{C}$ has the template of $\mathbb{S}$ and the deployment process is unnoticeable for the users.}  
In the constructor, $\mathcal{R}$ with $PK_\mathbb{U}$ are stored and ID of $\mathbb{S}$ (i.e., $\mathbb{S}^{ID}$) is assigned by a blockchain platform and returned in a response.\footnote{Note that $\mathbb{S}^{ID}$ represents a public identification of $\mathbb{S}$, which serves as a destination for sending crypto-tokens to $\mathbb{S}$ by any party.}
% \footnote{... E.g., in Ethereum~\cite{wood2014ethereum}, $\mathbb{S}^{ID}$ is represented by an address of $\mathbb{S}$ and is computed in a deterministic way using $PK_\mathbb{U}$ and the number of transactions executed by $\mathbb{U}$.}
%
Storing $\mathcal{R}$ and $PK_\mathbb{U}$ binds an instance of $\mathbb{S}$ with the user's authenticator $\mathbb{A}$ and the user's private key wallet $\mathbb{W}$, respectively. 
In detail, $PK_\mathbb{U}$ enables $\mathbb{S}$ to verify whether an arbitrary transaction was signed by the user who created $\mathbb{S}$, while $\mathcal{R}$ enables the verification whether the given OTP was produced by the user's $\mathbb{A}$.
%



\subsubsection{\textbf{Operation Execution}}
When the wallet framework is initialized, it is ready for executing operations by a two-stage protocol $\Pi_{O}$ (see \autoref{fig:smart-contract-execution} and Appendix~\ref{appendix:protocols}): 
%
\begin{figure}[t]
	\begin{center}
		\vspace{-0.4cm}
		\includegraphics[width=0.44\textwidth]{fig/deploy-scheme-bw.pdf} 
		\caption{Bootstrapping of SmartOTPs in a secure environment ($\Pi_{B}^\mathcal{S}$).}
		
		\label{fig:smart-contract-deploy}
		\vspace{-0.1cm}
	\end{center}	
\end{figure}
%
\begin{compactenum}
    \item \textbf{Initialization Stage}.
	When $\mathbb{U}$ decides to execute an operation with SmartOTPs, he enters the details of the operation into $\mathbb{C}$ that creates a transaction calling \textit{initOp()}, which is provided with operation-specific parameters -- the type of operation (e.g., transfer), a numerical parameter (e.g., amount or daily limit), and an address parameter (e.g., recipient). 
	Then, $\mathbb{C}$ sends this transaction to $\mathbb{W}$, which displays the details of the transaction and prompts $\mathbb{U}$ to confirm signing by a hardware button.
	Upon confirmation, $\mathbb{W}$ signs the transaction by $SK_{\mathbb{U}}$ and sends it back to $\mathbb{C}$.
%	\footnote{We require $\mathbb{W}$ to be a hardware wallet with display  (e.g., \cite{trezor-hw-wallet,ledger-nano-s,keep-key,BitLox,ellipal-hw-wallet}), enabling $\mathbb{U}$ to verify the details of transactions being signed.} 
	%
	$\mathbb{C}$ forwards the transaction to $\mathbb{S}$. % deployed at the blockchain.
	In the function \textit{initOp()}, $\mathbb{S}$ verifies whether the signature was created by $\mathbb{U}$ (the first factor), stores the parameters of the operation, and then assigns a sequential ID (i.e., $opID$) to the initiated operation.
	In the response from $\mathbb{S}$, $\mathbb{C}$ is provided with an $opID$.



\item \textbf{Confirmation Stage}.
    After the transaction (that initiated the operation) is persisted on the blockchain, $\mathbb{U}$ proceeds to the second stage of $\Pi_{O}$.
    %
%	To further protect our scheme against the attacker that tampers with the client (i.e., displaying different details of the operation from the blockchain's data), it is important to verify the details of the operation by other means than the client.   
%	For example, the user may use the HTTPS blockchain explorer, where the transaction details are displayed.
%	Since the client is a decentralized application, another option is to use a watch-only instance of the client on a smartphone or any other device. 
	%
	$\mathbb{U}$ enters $opID$ to $\mathbb{A}$, which, in turn, computes and displays $OTP_{opID}$ as $F_k(opID)$.
    %
    Storing $hOTPs$ computed from OTPs at $\mathbb{C}$ enables $\mathbb{U}$ to transfer only the displayed OTP from $\mathbb{A}$ to $\mathbb{C}$, which can be accomplished in an air-gapped manner. 
    Considering the mnemonic implementation~\cite{bipMnemonic}, this means an air-gapped transfer of 12 words in the case of $O=\text{16B}$.
%\footnote{Note that mnemonic bytes-to-string and string-to-bytes conversions can be presented as a part of the authenticator and the client, while the client can communicate with the smart contract using raw data only -- not requiring expensive computations for such conversions at the smart contract.}
    %
    Then, $\mathbb{C}$ computes and appends the corresponding proof $\pi_{opID}$ to the OTP.
    The proof of the OTP is computed from stored $hOTPs$ in the $\mathbb{C}$'s storage (or directly fetched from the storage if $\mathbb{C}$ stores all nodes of the Merkle tree).
    %
    Next, $\mathbb{C}$ sends a transaction with $OTP_{opID}$ and its proof $\pi_{opID}$ to the blockchain, calling the function \textit{confirmOp()} of $\mathbb{S}$, which handles the second factor. 
    This function verifies the authenticity of the OTP (i.e., the first requirement of OTPs) and its association with the requested operation (i.e., the second requirement of OTPs), which together implies the correctness of the provided OTP.\footnote{Note that SmartOTPs meet the third requirement of OTPs by the design.}
	%
    In detail, upon calling the \textit{confirmOp()} function with $opID$, $OTP_{opID}$, and $\pi_{opID}$ as the arguments, $\mathbb{S}$ reconstructs the root hash from the provided arguments by the function \textit{deriveRootHash()} that is presented in Appendix~\ref{appendix:algs}.\footnote{Note that this algorithm contains, not yet described, improvements.}
    %
    If the reconstructed value matches the stored value $\mathcal{R}$, the operation is executed (e.g., crypto-tokens are transferred).
    
    %
%    In this function, first a check of the correct length of $\pi_{opID}$ is made in order to avoid a second pre-image attack on $\mathcal{R}$.
%    %
%    Second, an OTP index is derived from $\pi_{opID}$,\footnote{Note that each item of the proof dedicates one bit to indicate the left/right position of this item in the Merkle tree, enabling us to derive the $opID$.} 
%	and then the derived index is compared with the index of an operation that $\mathbb{U}$ passed in the arguments (i.e., \textit{opID}).
%	%
%    If this check is successful, then $\mathcal{R}$ is reconstructed and compared with the expected $\mathcal{R}$ in the calling function \textit{verifyOTP()}.  %from \autoref{alg:wallet-overview}.
%    In the positive case, the operation is executed (e.g., crypto-tokens are transferred).
    %
%    \begin{algorithm}
%    	\footnotesize{
%    		\caption{Compute $\mathcal{R}$ from OTP and its proof}\label{alg:MT-deriveRH} 
%    		\begin{algorithmic}[1]
%    			\Function{deriveRootHash}{$otp$, $proof$, $opID$} \textbf{private}
%    			\State \textbf{assert}($proof.len == H$)  \Comment{$H == log_2(N)$} 
%    			\State \textbf{assert}(opID == deriveIdx(proof))
%    			\State res = h(otp) %\Comment{$cm[0] \text{ == } OTP_{opID}$}
%    			\For{$\{i = 0; ~i < proof.len; ~\plusplus{i}\}$}
%    			\If{1 == LSB(proof[i])} 
%    			\State res  = h(res $\|$ proof[i])   \Comment{$proof[i]$ is on the right}
%    			\Else
%    			\State res  = h(proof[i] $\|$ res)  \Comment{$proof[i]$ is on the left}
%    			\EndIf
%    			\EndFor
%    			\State \Return res
%    			\EndFunction				  
%    			
%    			\Function{deriveIdx}{proof} \textbf{private}
%    			\State idx = 0
%    			\For{$\{i = 0; ~i < proof.len ; ~\plusplus{i}\}$}
%    			\If{1 == LSB(proof[i])}
%    			\State idx = idx $\mathrel{|}$ (1 $\ll$ i)
%    			\EndIf                        		
%    			\EndFor				         
%    			\State \Return idx		
%    			\EndFunction				  		
%    		\end{algorithmic}
%    	}
%    \end{algorithm}
    %
\end{compactenum}
%

\begin{figure}[t]
	\begin{center}
		\vspace{-0.4cm}
		\includegraphics[width=0.47\textwidth]{fig/operation-scheme-bw.pdf} 
		\caption{Execution of an operation ($\Pi_{O}$).}
		\label{fig:smart-contract-execution}		
	\end{center}	
	\vspace{-0.1cm}
\end{figure}




%The core functionality of the proposed smart-contract wallet is presented in \autoref{alg:wallet-overview}.
%
%Upon construction of the smart contract, the owner's address and $\mathcal{R}$ are stored on the block\-chain.
%Since that moment onward, the smart contract verifies either the sender of the transaction or the OTP provided, according to the stage of the proposed protocol.

%, and executes the operation of these two authentication steps successfully. 
%
%\feedback{[Why to drop it? this is important.] We emphasize that new operations can be added to the smart contract by extending the enum \textit{OpType} and the function \textit{execOp()}.
%We give examples of such operations in \autoref{sec:functionality-extension}.}

%\smallskip 
\noindent
In the following, we present extensions of SmartOTPs, improving its efficiency and usability, and introducing new features.
%\feedback{IH: i would like to distinguish between improvements and extension, as extension deals with extending operation sets.}
%See \autoref{fig:overview} for an overview of our approach enriched with all the proposed extensions.

%Notice that so far we abstracted ourselves from practical issues of this approach, such as the limited number of OTPs, possibly high operational costs, and other important usability issues.
%All of these issues will be detailed and addressed in the following.

\subsection{\textbf{Bootstrapping in an Insecure Environment}}\label{sec:bootstraping-insec}
The main advantage of $\Pi_{B}^\mathcal{S}$ described above is its high usability, requiring only an air-gapped transfer of $k$ and connected $\mathbb{W}$.
%
However, $\Pi_{B}^\mathcal{S}$ is not resistant against $\mathcal{A}$ tampering with $\mathbb{C}$; $\mathcal{A}$ might intercept $k$ or forge $\mathcal{R}$ for $\mathcal{R}'$.
Similarly, $\mathcal{A}$ might forge $PK_\mathbb{U}$ for $PK_\mathcal{A}$, while staying unnoticeable for $\mathbb{U}$ who expects that $\mathbb{S}^{ID}$ obtained is correct.
%
Therefore, we propose an alternative bootstrapping protocol $\Pi_{B}^\mathcal{I}$ (see Appendix~\ref{appendix:protocols}), assuming that $\mathcal{A}$ can tamper with $\mathbb{C}$ during bootstrapping.
%
In this protocol, first we protect SmartOTPs from the interception of $k$ and then from forging $\mathcal{R}$ and $PK_\mathbb{U}$. % with malicious values. 


To avoid the interception of $k$, instead of transferring $k$, $\mathbb{U}$ performs a transfer of all leaves of the Merkle tree (i.e., $hOTPs$) from $\mathbb{A}$ to $\mathbb{C}$, which can be achieved with a microSD card.
Note that the leaves are hashes of OTPs, hence they do not contain any confidential data.
%
Next, to protect SmartOTPs from forging of $PK_\mathbb{U}$ and $\mathcal{R}$,
we require a deterministic computation of $\mathbb{S}^{ID}$ by a blockchain platform using $PK_\mathbb{U}$ and $\mathcal{R}$, hence $\mathbb{S}^{ID}$ can be computed and displayed together with $\mathcal{R}$ in $\mathbb{W}$ before the deployment of $\mathbb{S}$.
In detail, $\mathbb{S}^{ID}$ is computed as $h(PK_\mathbb{U} ~\|~ \mathcal{R})$, thus each pair consisting of a public key and a root hash  maps to the only $\mathbb{S}^{ID}$.
%
However, even with this modification, $\mathcal{R}$ can still be forged by $\mathbb{C}$. 
Therefore, when transaction with the constructor is sent to $\mathbb{W}$, $\mathbb{U}$ has to compare $\mathcal{R}$ displayed at $\mathbb{W}$ with the one computed and displayed by $\mathbb{A}$. 
In the case of equality, $\mathbb{U}$ records $\mathbb{S}^{ID}$ displayed in $\mathbb{W}$. % while he can be sure that $\mathbb{S}^{ID}$ is associated with legitimate $PK_\mathbb{U}$ and $root$.
%\setlength{\textfloatsep}{0.1cm}
%\setlength{\floatsep}{0.1cm}




%\paragraph{\textbf{Resistance Against the Attacker Models}}

%\subsection{Extension by Standard Security Means}
%In order to ensure $(2 + 1/1)$-step authentication of our approach, we add standard security features such as encryption passwords to both the authenticator and the client.

% \subsection{Security Discussion}
% Our proposed approach is resistant against the attacker model B) thanks to security properties of asymmetric cryptography used for signing transactions.
% A resistance of our approach against the attacker model A) is achieved by our proposed protocol, which must ensure that all requirements on OTPs are met.
% %In the case of the attacker model A), the proposed approach protects against misusing of the user's private key thanks to confirmation stage of the protocol, requiring an OTP from the authenticator that is owned by a user.
% %
% We remind that an attacker can intercept and modify transactions in both initialization and confirmation stages of the protocol.
% When the initialization stage of the protocol is attacked, the attack will be visible on the blockchain, hence the client can detect an unexpected modification and stop it before the confirmation stage. % only if the initial stage is as expected.
% When an attacker intervenes in the confirmation part of the protocol, the protection is achieved due to the linkage of the OTP with the operation in confirmation (i.e., the second requirement on OTPs).
% This means that the attacker cannot confirm other than user's initiated transfer with such an intercepted OTP.
% %\footnote{Therefore, we can eliminate check whether a \textit{confirmOp()} transaction is signed by an owner of the contract, while not losing on the security.}


==> sec/pre.tex <==
%Background
%Problem Definition
%- Clear and concise problem formulation
%- Present specific quality metric for evaluation
%Attacker Model
%Assumptions

%\paragraph{Cryptocurrency and Smart Contracts}
%\label{sec:smart-contracts-background}
We assume a generic cryptocurrency of which the blocks of records are stored in an ever-growing public distributed ledger called a \textit{blockchain}, which is by design resistant to modifications. 
In a blockchain, blocks are linked using a cryptographic hash function, and each new block has to be agreed upon by participants running a consensus protocol (i.e., \textit{miners}).
%
Each block may contain orders transferring crypto-tokens, application codes written in a platform-supported language, and the execution orders of such applications. 
These application codes are referred to as \textit{smart contracts} and can encode arbitrary processing logic (e.g., agreements). % written in the supported language.
Interactions between clients and the cryptocurrency system are based on messages called \textit{transactions}, which can contain either orders transferring crypto-tokens or calls of smart contract functions.
All transactions sent to a blockchain are validated by miners who replicate the state of the blockchain.
%To incentivize miners, blockchain platforms introduce reward and fee schemes.

\paragraph{Merkle Tree}\label{sec:MT-background}
A Merkle tree is a data structure based on the binary tree in which every leaf node contains a hash of a single data block, while every non-leaf node contains a hash of its concatenated children.
A Merkle tree enables efficient verification as to whether some data are associated with a leaf node by comparing the expected root hash of a tree with the one computed from a hash of the data in the query and the remaining nodes required to reconstruct the root hash (i.e., \textit{proof} or \textit{authentication path}).
The reconstruction of the root hash has logarithmic time complexity, which makes the Merkle tree an efficient scheme for membership verification.


%\paragraph{User Authentication}
%Authentication is a method of verifying the claimed identity of a user who requests access to a resource or a service.
%If an authentication method requires the user to present a combination of two or more distinct factors proving knowledge, possession, or inherent biometric features, we refer to multi-factor authentication (MFA).
%In practice, 2-factor authentication (2FA) is commonly used; this is a variant of MFA that requires proving two of mentioned factors -- usually knowledge and possession.
%%
%In order to break particular factors of MFA, the attacker must extract a knowledge factor (e.g., password), physically steal a device possessed by the user, and forge the user's biometric features, respectively.  
%%
%Multi-step authentication (MSA) is an authentication method that requires the user to present a combination of two or more instances of a single factor -- proving either knowledge, or possession, or inherent biometric features.
%The most common variant of MSA is 2-step authentication (2SA), which requires proving two instances of a knowledge factor (e.g., password, software-based OTP).
%%
%In contrast to MFA, breaking MSA requires the attacker to execute only a single type of malicious action, but multiple times in more contexts -- for example, extracting a password (e.g., by a keylogger) and extracting a private seed of an application generating OTPs (e.g., by malware).
%%
%Since terms MFA and MSA differ only in the realization of a particular step's/factor's data source (e.g., sealed hardware VS a software in the case of 2FA/2SA), we will further use only term MFA (or 2FA) for simplification of the terminology. 
%When needed we will distinguish between these two terms explicitly.

\subsection{Notation}\label{sec:notation}
%
% \setlength{\tabcolsep}{8pt}
% \begin{table}[b]
% 	\begin{center}
% 	% \renewcommand*{\arraystretch}{1.25}
% 	\begin{tabular}{rl}
% 		$\{msg\}_A$ & denotes the message $msg$ digitally signed by $A$, \\
% 		$h(.)$ & is a cryptographic hash function, \\
% 		$\|$ & is the string concatenation, \\
% 		$\oplus$ & represents bitwise XOR, \\
% 		%$r\xleftarrow{R}S$ & denotes $r$ is an element randomly selected from the set $S$,\\
% %		$\{0,1\}^n$ & is a set of all $n$-bit long strings
% 		%$t_x$ & is a Unix timestamp expressed in seconds. \\
% 	\end{tabular}
% 	\end{center}
% 	
%     \caption{Notation used throughout the paper.}
%     \label{tab:notation}
% \end{table}
% \setlength{\tabcolsep}{1.4pt}
%
By the term \textit{operation} we refer to an action with a smart-contract wallet using SmartOTPs, which may involve, for instance, a transfer of crypto-tokens or a change of daily spending limits.
%The operation is always performed in two steps, consisting of initialization and confirmation part.
%
Then, we use the term \textit{transfer} for the indication of transferring crypto-tokens. 
%either directly from a user to a recipient address (i.e., \textit{direct transfer}) or indirectly using the proposed wallet (i.e., \textit{authenticated transfer}).
%
%The term \textit{confirmation material} will be used for referring to the second-step-authenticated data (i.e., an OTP with its authentication path from Merkle tree).
%
%Finally, the term \textit{authenticator's public key} will be used for referring to the root hash of a Merkle tree, which publicly identifies an instance of the authenticator and at the same time can be used for verification of whether a confirmation material was produced by a particular authenticator.
%
By $\{msg\}_\mathbb{U}$ we denote the message $msg$ digitally signed by $\mathbb{U}$, and by $msg.\sigma$ we refer to the signature;
%$B = \{0,1\}$ represents a set of bit values, while $B^+$ indicates positive iteration of set $B$, yielding a set of all bit strings;
%$h(l) ~|~ l\in A^*$
%$\mathbb{N}_0 = \{0, 1, 2, \ldots\}$;
$\mathcal{RO}$ is the random oracle;
$h(.)$: stands for a cryptographic hash function;
$h^i(.)$ substitutes $i$-times chained function $h(.)$, e.g., $h^2(.) \equiv h(h(.))$;
$\|$ is the string concatenation;
$h_{\mathcal{D}}^i(.)$ substitutes $i$-times chained function $h(.)$ with embedded domain separation, e.g., $h_{\mathcal{D}}^2(.) = h(2 ~||~ h(1~||~.))$;
%$GCD(A,B)$ is the greatest common divisor of $A$ and $B$;
$F_k(.) \equiv h(k ~\|~ .)$ denotes a pseudo-random function that is parametrized by a secret seed $k$;
$\%$ represents modulo operation over integers; 
$\Sigma. \{KeyGen, Verify, Sign\}$ represents a signature scheme of the blockchain platform;
$SK_\mathbb{U}$, $PK_\mathbb{U}$ is the private/public key-pair of $\mathbb{U}$, under $\Sigma$,
and $a~|~b$ represents bitwise OR of arguments $a$ and $b$.
%$\mathrel{|}$ represents logical OR; 


\section{Problem Definition}
The main goal of this work is to propose a cryptocurrency wallet framework that provides a secure and usable way of managing crypto-tokens. 
%
In particular, we aim to achieve:
\begin{compactdesc}
\item[Self-Sovereignty:] 
 ensures that the user does not depend on the 3rd party's infrastructure, and the user does not share his secrets with anybody.
 Self-sovereign (i.e., non-custodial) wallets do not pose a single point of failure in contrast to server-side (i.e., custodial) wallets, which when compromised, resulted in huge financial loses~\cite{2018-coindesk-bithumb,2014-Mt-Gox,2016-Bitfinex-hack,moore2013beware,binance-hack-2019}.
 %
% \red{The next argument for a self-sovereignty is the natural difference in user needs. 
% Cryptocurrency platforms offer native pre-defined security features that are available for all users. Unfortunately, these solutions lack expressiveness, as they have to fit standard users (who, e.g., store crypto-tokens as a hobby) as well as large cryptocurrency exchange providers, which, due to the value stored, require much better protection.}\ih{this is more customization than self-sovereingty}
 %
\item[Security:] the insufficient security level of some self-sovereign wallets has caused significant financial losses for individuals and companies~\cite{2016-brainwallets,courtois2016speed,CHHMPRSS18,parity-bug-July-17}. 
We argue that wallets should be designed with security in mind and in particular, we point out 2FA solutions, which have successfully contributed to the security of other environments~\cite{aloul2009two,schneier2005two}.
%
Our motivation is to provide a cheap security extension of the hardware wallets (i.e., the first factor) by using OTPs as the second factor in a fashion similar to Google Authenticator.   
%In the context of cryptocurrencies, we emphasize that implementing OTPs is challenging, as all blockchain data are public. 
%We see usability and cost benefits of an air-gapped setting, as it prevents from multiple attack vectors related to connected devices~\cite{bui2018man}. \ih{this is not true for hw wallets with display}
%
\end{compactdesc}

\vspace{-0.15cm}
\subsection{Threat Model}\label{sec:threat-model}
For a generic cryptocurrency described in \autoref{sec:pre}, we assume an adversary $\mathcal{A}$ whose goal is to conduct unauthorized operations on the user's behalf or render the user's wallet unusable. 
%(e.g., by an OTP depletion attack).
$\mathcal{A}$ is able to eavesdrop on the network traffic as well as to participate in the underlying consensus protocol. 
However, $\mathcal{A}$ is unable to take over the cryptocurrency platform nor to break the used cryptographic primitives.
We further assume that $\mathcal{A}$ is able to intercept and ``override'' the user's transactions, e.g., by launching a man-in-the-middle (MITM) attack or by creating a conflicting malicious transaction with a higher fee, which will incentivize miners to include $\mathcal{A}$'s transaction and discard the user's one; this attack is also referred to as \textit{transaction front-running}.
%
We assume three types of exclusively occurring attackers, each targeting one of the three components of our framework: (1) $\mathcal{A}$ with access to the user's private key hardware wallet, (2) $\mathcal{A}$ that tampers with the client, and for completeness we also assume (3) $\mathcal{A}$ with access to the authenticator.
%
%while our main focus is on the first attacker.
Next, we assume that the legitimate user correctly executes the proposed protocols and $h(.)$ is an instantiation of $\mathcal{RO}$. 
%and secrets are generated using~$\mathcal{RO}$.

\vspace{-0.15cm}
\subsection{Design Space}\label{sec:design-space}
There are many types of wallets with different properties (see Appendix~\ref{appendix-soa}).
In our context, to achieve self-sovereignty we identify smart-contract wallets as a promising category.
These wallets manage crypto-tokens by the functionality of smart contracts, enabling users to have customized control over their wallets. 
%(to the extend provided by a particular smart contract wallet). 
The advantages of these solutions are that spending rules can be explicitly specified and then enforced by the cryptocurrency platform itself.
% -- it is impossible to bypass them, as they are verified by miners.
Therefore, using this approach, it is possible to build a flexible wallet with features such as daily spending limits or transfer limits.
%

\paragraph{General OTPs}
With spending rules encoded in a smart contract, it is feasible to design custom security features, such as OTP-based authentication serving as the second factor. %, which is the goal of our work.
In such a setting, the authenticator produces OTPs to authenticate transactions in the smart contract.
%
However, in contrast to digital signatures,
%(such as RSA, DSA, Lamport signatures~\cite{lamport1979constructing-lamportSigs}, Merkle signatures~\cite{merkle1989certified}, Winternitz signatures~\cite{dods2005hash-winternitz}, etc.), 
OTPs do not provide non-repudiation of data present in a transaction with an OTP; moreover, they can be intercepted and misused by the front-running or the MITM attacks.
%
To overcome this limitation, we argue that a two-stage protocol $\Pi_O^{<G>}$ must be employed, enabling secure utilization of general OTPs in the context of blockchains.
In the first stage of $\Pi_O^{<G>}$, an operation $O$, signed by the user $\mathbb{U}$, is submitted to the blockchain, where it obtains an identifier $i$. 
Then, in the second stage, $O_{i}$ is executed on the blockchain upon the submission of $OTP_{i}$ that is unambiguously associated with the operation initiated in the first stage. 

\paragraph{Requirements of General and Air-Gapped OTPs}
Based on the above, we define the necessary security requirements of general OTPs used in the blockchain as follows:
\begin{compactenum}
	\item \textbf{Authenticity:} each OTP must be associated only with a unique authenticator instance. % and thus must allow the verification of the authenticity of an OTP.
	
	\item \textbf{Linkage:} each $OTP_{i}$ must be linked with exactly a single operation $O_i$, ensuring that $OTP_i$ cannot be misused for the authentication of $O_j, i \neq j$.
	%
	%	See \autoref{sec:details} for details about modification of the Merkle tree scheme, which ensures this security requirement.
	
	\item \textbf{Independence:} $OTP_i$ linked with the operation $O_i$
	cannot be derived from $OTP_j$  of an operation $O_j$, where $i \neq j$, or an arbitrary set of other OTPs. 	
\end{compactenum}
Nevertheless, in the air-gapped setting (important for a high usability and security), one more requirement comes into play: \textbf{the short length of OTPs}. 
Short OTPs allow the users to use a relatively small number of mnemonic words or a small QR code to transfer an OTP in an air-gapped fashion.
This requirement is of high importance especially in the case when the authenticator is implemented as a resource-constrained embedded device with a small display (e.g., credit-card-shaped wallet, such as CoolBitX~\cite{CoolWalletS}).

\paragraph{Analysis of Existing Solutions}
%
We argue that not all solutions meet the requirements of air-gapped OTPs.
%
Asymmetric cryptography primitives such as digital signatures or zero-knowledge proofs are inadequate in this setting, despite meeting all general OTP requirements.
State-of-the-art signature schemes with reasonable performance overhead~\cite{bernstein2012high,johnson2001elliptic} and short signature size produce a 48B-64B long output.
The BLS signatures~\cite{boneh2001short} go even beyond the previous constructs and might produce signatures of size 32B. 
Nevertheless, BLS signatures are unattractive in the setting of the smart contract platforms that put high execution costs for BLS signature verification, which is $\sim$33 times more expensive than in the case of ECDSA with the equivalent security level~\cite{RFC-BLS-signatures}.
Hence, we assume 48B as the minimal feasible OTP size for assymetric cryptography.

However, transferring even 48B in a fully air-gapped environment by transcription of mnemonic words~\cite{bipMnemonic} would lack usability for regular users -- considering study from Dhakal et al.~\cite{Dhakal-typing-study}, transcription of 36 English words takes 42s on average, which is much longer than users are willing to ``sacrifice.''
We note that the situation is better with QR code, but on the other hand it has two limitations: 
(1) when the authenticator is implemented as a simple embedded device, its display might be unable to fit a requested QR code with sufficient scanning properties (to preserve the maximal scanning distance of QR code, the ``denser'' QR code must be displayed in a larger image~\cite{QR2011size}) and 
(2) occasionally, the users might not have a camera in their devices, thus, they can proceed only with a fallback method that uses mnemonics.
%
%Another drawback of asymmetric cryptography relates to its resource demands that increase the operational costs, both on authenticators and on smart contracts (smart contract platforms put a high execution cost for asymmetric cryptography).
Finally, most of the currently deployed asymmetric constructions are vulnerable to quantum computing~\cite{bernstein2009introduction}.

The problem of long signatures also exists in hash-based signature constructs~\cite{lamport1979constructing-lamportSigs,dods2005hash-winternitz,merkle1989certified}. 
%such as Lamport-Diffie one-time Winternitz one-time signatures~\cite{dods2005hash-winternitz}, and Merkle signatures~\cite{merkle1989certified}. 
Lamport-Diffie one-time signatures (LD-OTS)~\cite{lamport1979constructing-lamportSigs} produce an output of length $2|h(.)|^2$, which, for example in the case of $|h(.)| = 16B$ yields $4kB$-long signatures. 
The signature size of LD-OTS can be reduced by using one string of one-time key for simultaneous signing of several bits in the message digest (i.e., Winternitz one-time signatures (W-OTS)~\cite{dods2005hash-winternitz}), but at the expense of exponentially increased number of hash computations (in the number of encoded bits) during a signature generation and verification.
The extreme case minimizing the size of W-OTS to $|h(.)|$ (for simplicity omitting checksum) would require $2^{|h(.)|}$ hash computations for signature generation, which is unfeasible. 

Approaches based on symmetric cryptography primitives produce much shorter outputs, but it is challenging to implement them with smart-contract wallets.
Widely used one-time passwords like HOTP~\cite{m2005hotp} or TOTP~\cite{m2011totp} require the user to share a secret key $k$ with the authentication server. 
Then, with each authentication request the user proves that he possesses $k$ by returning the output of an $F_k(.)$ computed with a nonce (i.e., HOTP) or the current timestamp (i.e., TOTP).
This approach is insecure in the setting of the blockchain, as the user would have to share the secret $k$ with a smart-contract wallet, making $k$ publicly visible. 

A solution that does not publicly disclose secret information and, at the same time, provides short enough OTPs (e.g., $16B \simeq 12$ mnemonic words $\simeq$ QR code v1), can be implemented by Lamport's hash chains~\cite{lamport1981password} or other single hash-chain-based constructs, such as T/Key~\cite{kogan2017t}.
A hash chain enables the production of many OTPs by the consecutive execution of a hash function, starting from $k$ that represents a secret key of the authenticator.
Upon the initialization, a smart contract is preloaded with the last generated value $h^n(k)$.
%
When the user wants to authenticate the $i$th operation, he sends the $h^{n-i}(k)$ to the smart contract in the second stage of $\Pi_O^{<G>}$. 
The smart contract then computes $h(.)$ consecutively $i$ times and checks to ascertain whether the obtained value equals the stored value. 
%
However, the main drawback of this solution is that \textit{each OTP can be trivially derived from any previous one}, and thereby this scheme does not meet the requirement of OTPs on independence. 
To detail an attack misusing this flaw, assume the MITM attacker possessing $SK_{\mathbb{U}}$ (i.e., the first factor) is able to initiate operations in the first stage of $\Pi_O^{<G>}$.
The attacker $\mathcal{A}$ initiates operation $O_i$ and waits for $\mathbb{U}$ to initiate and confirm an arbitrary follow-up operation $O_j, j > i$. 
When $\mathbb{U}$ sends $OTP_j$ in the second stage of $\Pi_O^{<G>}$, $\mathcal{A}$ intercepts and ``front-runs'' the user's transaction by a malicious transaction with $OTP_i$ computed as $h^{j-i}(OTP_j)$.
%
Although one may argue that this scheme can be hardened by a modification denying to confirm older operations than the last initiated one, it would bring a race condition issue in which $\mathcal{A}$ might keep initiating operations in the first stage of $\Pi_O^{<G>}$ each time he intercepts a confirmation transaction from $\mathbb{U}$, causing the DoS attack on the wallet.

%As a consequence, ``selective confirmation'' of operations is impossible since revealing the $i$th OTP allows the attacker possessing $SK_{\mathbb{U}}$ to derive any $j$th OTP, where $j<i$.



%In order to defend Lamport's hash chain against attacker A),  a modification denying to confirm older operations than the last confirmed operation can be applied.
%However, the modification fails to defend this OTP scheme against the attacker model B), as the attacker can intercept and steal the OTP, compute one or a few steps of a hash chain in order to obtain OTP required by his operation.

%A solution that meets both requirements on OTPs and at the same time provides short enough OTPs can be realized using PRF for generating OTPs and Merkle tree for their aggregation.
%However, in contrast to digital signatures or Merkle tree signatures~\cite{merkle1989certified}, such OTPs are not tied to any data except an order of the operation, therefore 2-step authentication is more challenging in that setting.
%For instance, if an operation and its corresponding OTP are submitted to the blockchain in a single stage, an attacker can block this action, create a fake operation and use stolen OTP to authenticate his operation.
%To prevent this issue, we propose a two-stage approach, where an operation is first submitted to the blockchain and then in the second stage it is executed upon authentication by the corresponding OTP.
%}







==> sec/related.tex <==
In this section, we compare SmartOTPs with other hash-based approaches and other smart-contract wallets.
%then we propose a classification of blockchain-related authentication schemes,
%Then, we extend the previous work of Eskandari et al.~\cite{eskandari2018first} and Bonneau et al.~\cite{2015-Bitcoin-SOK}, by categorizing and reviewing examples of cryptocurrency wallet solutions.
For an overview of existing wallet solutions, we refer the reader to  Appendix \ref{sec:classification} and \ref{sec:soa-wallet-types}, where we apply and extend the categorization of Eskandari et al.~\cite{eskandari2018first} and Bonneau et al.~\cite{2015-Bitcoin-SOK}.



\paragraph{\textbf{Hash-Based Approaches}}\label{sec:related-comparison}
Although Merkle signatures~\cite{merkle1989certified} utilize Merkle trees for aggregation of several one-time verification keys (e.g.,~\cite{lamport1979constructing-lamportSigs}), the size of these keys and signatures is substantially larger than the size of OTPs in Smart\-OTPs.
Even further optimization of the signature size (i.e., Winternitz OTS~\cite{dods2005hash-winternitz}) does not make signatures as short as in SmartOTPs.
%
Next, we highlight that we utilize hash chains for multiplication of OTPs, which is different than their application in Winternitz OTS~\cite{dods2005hash-winternitz} that utilize them for the purpose of reducing the size of a single Lamport-Diffie OTS~\cite{lamport1979constructing-lamportSigs} by encoding multiple bits of a message digest into the number of recurrent hash computations.
%
The next related schemes are Lamport's hash chain~\cite{lamport1981password} and its modification T/Key~\cite{kogan2017t} that applies the domain separation.
However, since they contain only a single chain, they are not secure in the setting of the public blockchain (see \autoref{sec:design-space}) in contrast to SmartOTPs that never consecutively iterate OTPs within a single hash chain.
%
Moreover, T/Key~\cite{kogan2017t} is using OTPs expiring in 30s to mitigate phishing attacks, which are unrelated in our case.
%SmartOTPs protects against such an attack by protocol with 2 stages. 
TESLA~\cite{perrig2000efficient,perrig2005rfc4082} is another related scheme that utilizes a single hash-chain in a centralized setting of time-based multi-cast authentication of streamed messages.

\begin{figure}[t]
	\centering
	\vspace{-0.3cm}
	
	\includegraphics[width=0.35\textwidth]{fig/cost-new-subtree.pdf} 	
	\vspace{-0.2cm}
	
	\caption{Cost of introducing the next subtree ($H = 20,~ H_S = 10$).}\label{fig:cost-of-new-subtree}
	%		\vspace{-0.1cm}
\end{figure}



%The problem of long signatures exists also in hash-based signature constructs~\cite{lamport1979constructing-lamportSigs,dods2005hash-winternitz,merkle1989certified}. 
%%such as Lamport-Diffie one-time Winternitz one-time signatures~\cite{dods2005hash-winternitz}, and Merkle signatures~\cite{merkle1989certified}. 
%Lamport-Diffie one-time signatures (LD-OTS)~\cite{lamport1979constructing-lamportSigs} produce output of length $2|h(.)|^2$, which, for example in the case of $|h(.)| = 16B$ implies $4kB$-long signatures. 
%The signature size of LD-OTS can be reduced by using one string of one-time key for simultaneous signing of several bits in the message digest (i.e., Winternitz one-time signatures (W-OTS)~\cite{dods2005hash-winternitz}) but at the expense of exponentially increased number of hash computations (in the number of encoded bits) during a signature generation and verification.
%The extreme case minimizing the size of W-OTS to $|h(.)|$ (for simplicity omitting checksum) would require $2^{|h(.)|}$ hash computations for signature generation, which is unfeasible. 

\begin{figure*}[t]
	\centering	
	\vspace{-0.6cm}
	
	\subfloat[\label{fig:fig:MT-current-benefit-of-caching-256} $H = 8$]{
		\hspace{-0.25cm}
		\includegraphics[width=0.30\textwidth]{fig/payoff-caching-B16-256.pdf} 
	}
	\subfloat[\label{fig:fig:MT-current-benefit-of-caching-512} $H = 9$]{
		\hspace{-0.25cm}
		\includegraphics[width=0.30\textwidth]{fig/payoff-caching-B16-512.pdf} 
	}
	\subfloat[\label{fig:fig:MT-current-benefit-of-caching-1024} $H = 10$]{
		\hspace{-0.25cm}
		\includegraphics[width=0.30\textwidth]{fig/payoff-caching-B16-1024.pdf} 
	}
	
	\vspace{-0.4cm}
	\caption{Rolling average cost per transfer ($H = H_S$).}
	\label{fig:MT-current-benefit-of-caching}
	\vspace{-0.5cm}	
\end{figure*}
\begin{figure*}[t]
	\centering
	
	\vspace{-0.1cm}
	\hspace{-0.5cm}	
	
	\subfloat[\label{fig:expenses-hash-chain-optim}$L = H$]{
		\hspace{-0.25cm}
		\includegraphics[width=0.30\textwidth]{fig/expenses-hash-chains-optim.pdf} 
	}
	\subfloat[\label{fig:expenses-hash-chain-maxCache}$L = 7$]{
		\hspace{-0.25cm}
		\includegraphics[width=0.285\textwidth]{fig/expenses-hash-chains-max.pdf} 
	}
	\subfloat[\label{fig:expenses-hash-chain-zero-cache}$L = 0$]{
		\hspace{-0.25cm}
		\includegraphics[width=0.285\textwidth]{fig/expenses-hash-chains-zero.pdf} 
	}	
	

	\hspace{1.5cm}
	\vspace{-0.4cm}	
	\caption{Average total cost per transfer with regards to the length $P$ of hash chains.}
	\vspace{-0.3cm}	
	\label{fig:hash-chain-expenses}
\end{figure*}

\paragraph{Smart Contract Wallets}
An example of the 2-of-3 multi-signature approach that only supports Trezor wallets is \textit{TrezorMultisig2of3}~\cite{TrezorMultisig2of3}.
A disadvantage of this solution is that $\mathbb{U}$ has to own three Trezor devices, which might be an expensive solution. % that, moreover, relies only on a single vendor.
%N-of-m multi-signature is  Parity Wallet~\cite{parity-wallet}. 
%However, two critical bugs~\cite{parity-bug-July-17,parity-bug-November-17} have caused the multi-signature scheme to be currently disabled.
%
% I skipped BitGo~\cite{BitGo-MultiSigWallet}, which is also 2-of-3
%
The n-of-m multi-signature scheme is provided by \textit{Gnosis Wallet}~\cite{ConsenSys-gnosis}, which currently holds a significant amount of Ether across various smart contracts.
Similar to the previous example, a disadvantage of this wallet is that $\mathbb{U}$ has to own two hardware wallets for 2FA.


The main reason why existing smart contract wallets using asymmetric cryptography are not suitable for an air-gapped authentication is due to the signature size of 64B.
Hence, to input OTP, $\mathbb{U}$ has to transcribe 48 mnemonic words in the case of lacking a camera on $\mathbb{C}$, which would take $\sim$4x longer than in the case of SmartOTPs.
When $\mathbb{C}$ is equipped with a camera, $\mathbb{A}$ implemented as an embedded device might not be capable of displaying a single OTP as a small QR code since the minimal required QR code having enough data capacity is v4. % which contains 33x33 modules. 
Therefore, several QR codes of a lower version would be needed, which introduces additional complexity for $\mathbb{U}$.
%


Another drawback of asymmetric cryptography (used in these wallets) stems from its resource demands that increase the operational costs, both on $\mathbb{S}$ and $\mathbb{W}$: 
(1) smart contract platforms place a high execution cost for asymmetric cryptography, and 
(2) $\mathbb{W}$ requires more advanced MCU for cryptographic computations, while $\mathbb{A}$ from SmartOTPs requires only a secure hash function. 
Based on the latter, we believe that hardware realization of $\mathbb{A}$ (see Appendix~\ref{appendix:NodeMcu-schema}) in SmartOTPs is less expensive than the second hardware wallet used in multi-signature smart contracts. 
Moreover, we note that if SmartOTPs were to use only mnemonic words and omit QR codes, then hardware requirements of $\mathbb{A}$ (and thus the overall cost) would be even lower -- mnemonic words can be displayed even on a smart-card-embedded display, such as in CoolBitX~\cite{CoolWalletS}.
%
%Finally, asymmetric constructions used in these wallets are less resilient to quantum computing attacks~\cite{bernstein2009introduction} than SmartOTPs \ih{Quantify}.


%1) asymmetric cryptography has weaker quantum resilience than hash-based cryptography in SmartOTPs, 
%2) asymmetric cryptography requires more advanced HW-chips for computations within *A*, while SmartOTPs require only a secure hash function, 
%3) based on the previous and Answer\_A1, we believe that HW realization of *A* is less expensive than in the case of 2 HW wallets with multisig.



==> sec/reviews-SP.tex <==

\subsection{Review $\#$900A}
\paragraph{\textbf{Overall merit}}
Reject - This paper is well below the bar for Oakland.  Will argue to reject it.

\paragraph{Brief paper summary}
This paper describes a solution for two-factor authentication (2FA) for blockchain transactions. 
In the context of blockchains, the verifier is a public smart contract, so a two-factor verification process cannot rely on secrets. 
The authors use a combination of PRFs, Merkle trees, and hash chains to produce a scheme for generating and verifying one-time authentication tokens.

\paragraph{Strengths}
\begin{compactenum}
	\item[S1] Well-motivated problem: 2FA is a standard measure for improving security in most traditional systems, so enabling 2FA for blockchain transactions seems natural.
	
	\item[S2] The proposal incurs lower communication costs than public-key signature schemes and consumes less gas on Ethereum compared to alternate solutions.
	
	\item[S3] The paper is generally well-written.	
\end{compactenum}


\paragraph{Weaknesses}
\begin{compactenum}
	\item[W1] The solution is a straightforward combination of PRFs, Merkle trees, and hash chains to create one-time authentication tokens. PRFs are commonly used for 2FA in centralized settings; the use of hash chains for authentication without storing secrets dates back to 1981.
	
	\item[W2] Unclear if the solution is significantly better than alternative solutions that are much simpler and require far less state on the client initiating transactions.		
\end{compactenum}

\paragraph{Detailed comments for the author(s)}
\begin{compactenum}
	\item[C1] Although SmartOTPs incur lower communication costs (from the authenticator device to the client) than public-key signature schemes, the savings is only 4x. 
	
	\item[C2] Furthermore, the overall data sent to the blockchain is much larger in the case of SmartOTPs (because of loga\-rith\-mic-sized Merkle inclusion proofs) than a public key signature scheme (which only requires only 64 bytes). 
	Why is it a reasonable trade-off?
	
	\item[C3] "...  When $\mathbb{C}$ is equipped with a camera, $\mathbb{A}$ realized as an embedded device might not be capable of displaying a single OTP as a small QR code since
	the minimal required QR code having enough data capacity is v4" => Cound't the air-gapped device display multiple QR codes? 	
\end{compactenum}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Review $\#$900B}
\paragraph{\textbf{Overall merit}}
Weak accept - While flawed, the paper has merit and we should consider accepting it.


\paragraph{Brief paper summary}
The paper studies an interesting research question, that of enabling OTP 2FA for blockchain accounts where it is the blockchain/smart contract that verifiers the OTP as the 2FA.  
This is interesting because the smart contract cannot store any secrets, and standard digital signatures are not great because they are too long for being air-gapped and memorized by user or captured using QR codes.

\paragraph{Detailed comments for the author(s)}
\begin{compactenum}
	\item[C1] The authors design a hash-based signatures scheme that combines PRFs, hashing and Merkle trees to satisfy all the requirements. 
	The idea is cute. 
	There isn't anything specifically novel about the building blocks, but I don't recall having seen this exact combination to satisfy this specific requirements before, though I would not say it is a big leap in innovation to do so.
	
	\item[C2] The nice thing about the paper is that of clearly discussing the requirements which is bit unique, and how existing approaches don't quite work or don't meet the efficiency or security requirements. 
	It is also nice to see a full implementation and performance evaluation of the end-to-end system on the Ethereum platform. 
	
	\item[C3] I was surprised that the authors did not cite TESLA: \url{https://tools.ietf.org/html/rfc4082}; a hash-chain based standard for generating OTPs though a work similar to that was discussed.
	
	\item[C4] Overall, I found the work well-done and valuable. 
	It introduces and provides solution to an interesting practical problem in the blockchain space.
\end{compactenum}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Review $\#$900C}
\paragraph{\textbf{Overall merit}}
Weak accept - While flawed, the paper has merit and we should consider accepting it.

\paragraph{Brief paper summary}
This paper describes a 2FA method that works with an airgapped
authenticator, hardware wallet and a smart contract to manage
cryptocurrency tokens. It makes use of merkle trees and hash chains,
while separating the proofs from the one-time password in order to
minimize the amount of data the user has to move from the
authenticator to the client.

\paragraph{Strengths}
\begin{compactenum}
	\item[S1] Good insight that you can separate the proofs from the OTPs.
	
	\item[S2] This seems practical to implement and 2FA is important and useful in this context.
	
	\item[S3] Thorough analysis and evaluation.	 	 
\end{compactenum}


\paragraph{Weaknesses}
\begin{compactenum}
	\item[W1] The paper is a bit hard to understand and could be better organized.
	
	\item[W2] It's unclear to me how to recover if the user loses access to the authenticator.	
\end{compactenum}


\paragraph{Detailed comments for the author(s)}
\begin{compactenum}
	\item[C1] I am unclear on what ``against the blockchain'' means.
	
	\item[C2] The source code link leads to a 404.
	
	\item[C3] What is the recovery mechanism if the user loses access to the authenticator?
\end{compactenum}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
\section{Response to Reviews}

\subsection{Review $\#$900A}
\paragraph{W1} 
A combination of these primitives has never been used before in both centralized and decentralized settings.
%
Although the reviewer argues that use of hash-chains for authentication in centralized setting has begun in early 80's,  there are approaches utilizing them much later, e.g., TESLA~\cite{perrig2005rfc4082} in 2005 and T/Key~\cite{kogan2017t} in 2017; while hash-chains have never been utilized in a decentralized setting.
%
We emphasize that a single hash-chain cannot be directly utilized as 2FA scheme in decentralized setting due to front-running or DOS attacks (see the last 2 paragraphs in \autoref{sec:design-space}). 
SmartOTPs primarily utilize hash-chains as an extension that multiplies the number of OTPs (see \autoref{sec:increasingNoOfOTPs}), and moreover, SmartOTPs can work without hash-chains as well.
Also note that a hash-chain proposed in early 80's is vulnerable to birthday attacks, and it was improved by domain separation~\cite{leighton1995large,kogan2017t}.


\paragraph{W2} 
We have already made a comparison of SmartOTPs with other multi-sig wallets in terms of an air-gapped setting, cost of hardware, and operational costs (see \autoref{sec:related} and \autoref{sec:discusion}).
%
Also, the only state that is required to be stored by $\mathbb{C}$ is the cache of OTP hashes $hOTPs$ from the first iteration layer. 
This state can be computed anytime from seed $k$ or transferred by microSD card from $\mathbb{A}$ to $\mathbb{C}$ (see \autoref{sec:bootstraping-sec} and \autoref{sec:bootstraping-insec}).

\paragraph{C1} We are not aware of any other approach that would achieve better savings for arbitrary target security.

\paragraph{C2} This is only true for the base version that contains purely the Merkle tree (see \autoref{sec:base-version}) and requires $H$ items of the proof to be contained in the transaction.
However, with the extension that introduces caching of $L$th layer of the Merkle tree at $\mathbb{S}$ (see \autoref{sec:caching-smart-contract}), the number of items in the proof are reduced to $H$ - $L$.
%
For example, in the case of $H=10$ and optimal caching (see \autoref{sec:costs-MK}) where $L=7$, only three items of the proof are required.
In this case, SmartOTPs consume ~68B of transaction data (assuming 4B for operation ID and 128 bits for the size of $h(.)$), which is similar to asymmetric cryptography used in most of the blockchains.

\paragraph{C3} We note that the reviewer is quoting the text snippet from related work, where we talk about using asymmetric cryptography in an air-gapped 2FA setting, requiring transfer of 64B data by a QR code.
In response to the question raised, we agree that it is possible to display multiple QR codes on the embedded device but in the accompanied text we add on that this would impose additional complexity for the user.



\subsection{Review $\#$900B}

\paragraph{C1}
Although the primitives used in SmartOTPs are well-known, they have never been used for the purpose of 2FA in decentralized setting.

\paragraph{C3}
We updated the related work with TESLA~\cite{perrig2000efficient,perrig2005rfc4082} paper.


\subsection{Review $\#$900C}

\paragraph{W1}
We improved the organization of the paper.
Furthermore, to simplify practical understanding of our approach, we recorded several videos of our implementation and made them available through a Dropbox link.

\paragraph{W2 \& C3}
When $\mathbb{A}$ is initialized, $\mathbb{U}$ stores a secret seed $k$ as a recovery phrase (see \autoref{sec:overview}). 
%
If $\mathbb{U}$ losses access to $\mathbb{A}$, he can initialize a new instance of $\mathbb{A}$ from the backup of seed $k$.
Moreover, if $\mathbb{U}$ losses access to $\mathbb{A}$ and $\mathbb{W}$ at the same time (including their recovery seeds), he can still recover the funds with the last resort functionality (see \autoref{sec:implementation} and Appendix \ref{sec:functionality-extension}).

\paragraph{C1}
By authentication ``against'', we mean authentication of the user to the data stored at the blockchain with a private key/secret.

\paragraph{C2}
We believe that it was just a temporary outage of the Dropbox link since other reviewers did not complain about this. 


\subsection{Changes Made}
To address the comments of reviewers, we have made several changes.
In detail, we extended the discussion section by explicitly addressing: (1) the loss of secrets, (2) the state at the client, and (3) transaction size.
%
Next, we included TESLA in the related work and also improved the organization of the paper.

In addition to points mentioned in reviews, we included a detailed overview of existing wallets categories in Appendix, and we classified them using our simple proposed method.
Next, we made a proof-of-concept hardware implementation of SmartOTPs and placed the details into Appendix~\ref{appendix:NodeMcu-schema}.
Also, we enriched the Appendix by a detailed description of $\Pi_{ST}$, the protocol for introduction of the next subtree, and  $\Pi_{NR}^\mathcal{I}$, the protocol for introduction of a new parent tree in an insecure environment. 








 


==> sec/usability.tex <==
\ih{TBD Pieter}

==> sec/wallet-properties.tex <==


\subsubsection{\textbf{Classification and Properties of Wallets}}\label{appendix:classification}
\hfill

\noindent
We present a comparison of wallets and approaches from \autoref{sec:soa-wallet-types} in \autoref{tab:state-of-the-art}.
We apply our proposed classification on authentication schemes, while we also survey a few selected security and usability properties of the wallets from the work of Eskandri et al.~\cite{eskandari2018first}. 
In the following, we briefly describe each property and explain the criteria stating how we attributed the properties to particular wallets. 

\paragraph{\textbf{Air-Gapped Property}}
We attribute this property (Y) to approaches that involve at least one hardware device storing secret information, which do not need a connection to a machine in order to operate.
%All other approaches, including paper wallets lack this property (N).
%This property also denotes resilience against Man-in-the-Machine attackers~\cite{bui2018man}.

\paragraph{\textbf{Resilience to Tampering with the Client}}
We attribute this property (Y) to all hardware wallets that sign transactions within a device, while they require $\mathbb{U}$ to confirm transaction's details at the device (based on displayed information).
Then, we attribute this property to wallets containing multiple clients that collaborate in several steps to co-signs transactions (a chance that all of them are tampered with is low).
%
%We partially (P) attribute this property to approaches that do not implicitly provide the protection but instead require additional conditions to meet -- e.g., checking the state of the blockchain.

\paragraph{\textbf{Post-Quantum Resilience}}
We attribute this property (Y) to approaches that utilize hash-based cryptography that is known to be resilient against quantum computing attacks~\cite{amy2016estimating}.

\paragraph{\textbf{No Need for Off-Chain Communication}}
We attribute this property (Y) to approaches that do not require an off-chain communication/transfer of transaction among parties/devices
%\vfill
%\pagebreak
%\noindent 
to build a final (co-)signed transaction, before submitting it to a blockchain (applicable only for $Z \geq 2$ or $W_i \ge 2$). 


\paragraph{\textbf{Malware Resistance (e.g., Key-Loggers)}}
We attribute this property (Y) to approaches that either enable signing  transactions inside of a sealed device or split signing control over secrets across multiple devices. 

\paragraph{\textbf{Secret(s) Kept Offline}}
We attribute this property (Y) to approaches that keep secrets inside their sealed storage, while they expose only signing functionality.
Next, we attribute this property to paper wallets and fully air-gapped devices.

\paragraph{\textbf{Independence of Trusted Third Party}}
We attribute this property (Y) to approaches that do not require trusted party for operation, while we do not attribute this property to all client-side and server-side hosted wallets.
We partially (P) attribute this property to approaches requiring an external relay server for their operation.


\paragraph{\textbf{Resilience to Physical Theft}}
We attribute this property (Y) to approaches that are protected by an encryption password or PIN.
We partially (P) attribute this property to approaches that do not provide password and PIN protection but have a specific feature to enforce uniqueness of an environment in which they are used (e.g., bluetooth pairing). 

\paragraph{\textbf{Resilience to Password Loss}}
We attribute this property (Y) to approaches that provide means for recovery of secrets (e.g., a seed of hierarchical deterministic wallets).
%We partially attribute this property (P) to approaches that require an additional backup action to be performed beforehand.


\setlength{\tabcolsep}{2.0pt}
\begin{table*}[]
	\scriptsize{
		\vspace{-0.3cm}
		\begin{tabular}{lccccccccccccc}
			\toprule
			&
			\multicolumn{2}{c}{\specialcell{\textbf{Authentication Scheme}\\\\}} & \rotatebox[origin=l]{90}{\textbf{\specialcell{Air-Gapped Property}}} &
			\rotatebox[origin=l]{90}{\textbf{\specialcell{Resilience to Tampering\\ with the Client}}} &
			\rotatebox[origin=l]{90}{\textbf{\specialcell{Post-Quantum Resilience}}} &
			\rotatebox[origin=l]{90}{\textbf{\specialcell{No Need for Off-Chain\\Communication}}} &
			\rotatebox[origin=l]{90}{\textbf{\specialcell{Malware Resistance}}} &
			\rotatebox[origin=l]{90}{\textbf{\specialcell{Secret(s) Kept Offline}}} &
			\rotatebox[origin=l]{90}{\textbf{\specialcell{Independence of\\Trusted Third Party}}} &
			\rotatebox[origin=l]{90}{\textbf{\specialcell{Resilience to Physical Theft}}} &
			\rotatebox[origin=l]{90}{\textbf{\specialcell{Resilience to Password Loss}}} &
			\rotatebox[origin=l]{0}{\textbf{\specialcell{Comments}}} \\
			\expandafter\cline\expandafter{\expandafter2\string-3\smallskip}
			&
			\textbf{Classification} &
			\textbf{Details} &
			& & & & & & & & &  \\
			\toprule
			
			\smallskip
			\textbf{Keys in Local Storage}                       & $1 + (0)$          & Private key                                                   &                                               &                                                         &                                                   &                                                   &                                             &                                                  &                                                        &                                                       &                                                      &                                                                                                                  \\
			Bitcoin Core~\cite{BitcoinCore}                                & $1 + (0)$          & For one of the options                                                                      & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & Y                                                      & N                                                     & N/A                                                    &                                                                               \\
			MyEtherWallet~\cite{MyEtherWallet}                               & $1 + (0)$          &  For one of the options                                   & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & Y                                                      & N                                                     & N/A                                                    & \\
			\midrule
			\smallskip
			\textbf{Password-Protected Wallets}                  & $1 + (1)$          & \specialcell{Private key + encryption}                                  &                                               &                                                         &                                                   &                                                   &                                             &                                                  &                                                        &                                                       &                                                      & \\
			Armory Secure Wallet~\cite{Armory-SW-Wallet}                         & $1 + (1)$          &                                                                       & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & Y                                                      & Y                                                     & N                                                    &                                                                               \\
			Electrum Wallet~\cite{Electrum-SW-Wallet}                             & $1 + (1)$          &                                                                       & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & Y                                                      & Y                                                     & N                                                    &                                                                               \\
			MyEtherWallet (Offline)~\cite{MyEtherWallet}                     & $1 + (1)$          &                                                                       & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & Y                                                      & Y                                                     & N                                                    & \\
			Bitcoin Core~\cite{BitcoinCore}                                 & $1 + (1)$          &                                                                       & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & Y                                                      & Y                                                     & N                                                    & \\
			Bitcoin Wallet~\cite{BitcoinWallet}                                & $1 + (1)$          &                                                                       & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & Y                                                      & Y                                                     & N                                                    &\\
			\midrule
			\smallskip
			\textbf{Password-Derived Wallets}                    & $1 + (X_1)$         &                                                                       &                                               &                                                         &                                                   &                                                   &                                             &                                                  &                                                        &                                                       &                                                                                           &                                                                               \\
			Armory Secure Wallet~\cite{Armory-SW-Wallet}                         & $1 + (1)$          &                                                                       & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & Y                                                      & Y                                                     & Y                                                    & \\
			Electrum Wallet~\cite{Electrum-SW-Wallet}                             & $1 + (1)$          &                                                                       & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & Y                                                      & Y                                                     & Y                                                    & \\
			Metamask~\cite{MetamaskWallet}                             & $1 + (1)$          &                                                                       & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & Y                                                      & Y                                                     & Y                                                    & \\
			Daedalus Wallet~\cite{daedalus-wallet}                             & $1 + (2)$          & \specialcell{2 passwords}                                          & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & Y                                                      & Y                                                     & Y                                                    & \\
			\midrule
			\smallskip
			\textbf{\specialcell{Hardware Storage Wallets}}             &        $1 + (X_1)$        &                                                                       &                                               &                                                         &                                                   &                                                   &                                             &                                                  &                                                        &                                                                                                            &                                      &                                                                               \\
			Trezor~\cite{trezor-hw-wallet}                                      & $1 + (1)$          &                                                                       & N                                             & Y                                                       & N                                                 & Y                                                 & Y                                           & Y                                                & Y                                                      & Y                                                     & Y                                                    & \\
			Ledger~\cite{ledger-nano-s}                                     & $1 + (1)$          &                                                                       & N                                             & Y                                                       & N                                                 & Y                                                 & Y                                           & Y                                                & Y                                                      & Y                                                     & Y                                                    & \\
			KeepKey~\cite{keep-key}                                     & $1 + (1)$          &                                                                       & N                                             & Y                                                       & N                                                 & Y                                                 & Y                                           & Y                                                & Y                                                      & Y                                                     & Y                                                    & \\
			BitLox~\cite{BitLox}                                       & $1 + (2)$          &  2 passwords$^*$                                                                     & N                                             & Y                                                       & N                                                 & Y                                                 & Y                                           & Y                                                & Y                                                      & Y                                                     & Y                                                    & \specialcell{~$^*$Additionally, protection\\~~against the evil maid attack}                                      \\
			CoolWallet S~\cite{CoolWalletS}                       & $1 + (0)$          &                                                                       & N                                             & Y                                                       & N                                                 & Y                                                 & Y                                           & Y                                                & Y                                                      & P$^\dagger$                                                     & N/A                                                    & $^\dagger$\specialcell{Depending on the mode} \\
			
			Ledger Nano~\cite{ledger-nano}                                 & $1 + (2)$          &         Password + GRID card                                                               & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & Y                                                & Y                                                      & Y                                                     & Y                                                    & \\
			ELLIPAL wallet~\cite{ellipal-hw-wallet}                                      & $1 + (1)$          &                                                                       & Y                                             & Y                                                       & N                                                 & Y                                                 & Y                                           & Y                                                & Y                                                      & Y                                                     & Y                                                    & \\
			BitBox USB Wallet~\cite{BitBox}                          & $1 + (2)$          & 1 password and App                                                                       & N                                             & Y                                                       & N                                                 & Y                                                 & Y                                           & Y                                                & P$^\ddagger$                                                      & Y                                                     & Y                                                    & \specialcell{$^\ddagger$Requires a relay server}                \\
			
			\midrule
			\textbf{\specialcell{Split Control --\\Threshold Cryptography}}      & $1^{(W_1)} + (X_1^{1}, \ldots , X_1^{W_1})$         &                                                                       &                                               &                                                         &                                                   &                                                   &                                             &                                                  &                                                        &                                                       &                                                                                            &                                                                               \\
			Goldfeder et al.~\cite{goldfeder2015securing}                            & $1^{(2)} + (1,1)$   & \specialcell{Assuming 2 devices, each\\protected by a password}               & N                                             & Y                                                       & N                                                 & N                                                 & Y                                           & N/A                                              & N/A                                                    & N/A                                                     & N/A &                                                                               \\
			Mycelium Entropy~\cite{mycelium-entropy}                            & $1^{(2)} + (0,0)$   &                                                                       & N                                             & Y                                                       & N                                                 & N                                                 & Y                                           & Y                                                & Y                                                      & Y                                                     & N/A                                                    &                                                                               \\
			\midrule
			\smallskip
			\textbf{\specialcell{Split Control --\\Multi-Signature Wallets}}     & $Z + (X_1/\ldots/X_z)$    &                                                                       &                                               &                                                         &                                                   &                                                   &                                             &                                                  &                                                        &                                                                                                            &                                      &                                                                               \\
			\specialcell{Lockboxes of Armory\\Secure Wallet~\cite{Armory-SW-Wallet}}             & $Z + (X_1/\ldots/X_z)$    & $Z$ up to 7, $X_i$ = 1                                                     & N                                             & Y                                                       & N                                                 & N                                                 & Y                                           & N                                                & Y                                                      & Y                                                     & N                                                    & \\
			Electrum Wallet~\cite{Electrum-SW-Wallet}                             & $Z + (X_1/\ldots/X_z)$    & $Z$ up to 15, $X_i$ = 1                                                    & N                                             & Y                                                       & N                                                 & N                                                 & Y                                           & N                                                & Y                                                      & Y                                                     & Y                                                    & \\
			\specialcell{Trusted Coin's\\cosigning service~\cite{TrustedCoin-cosign}}            &     $2 + (1/2)$           & \specialcell{2 private keys + 2 passwords\\and Google Auth.} & N                                             & Y                                                       & N                                                 & N                                                 & Y                                           & N                                                & N                                                      & Y                                                     & Y                                                    & A hybrid client-side wallet                                                         \\
			Copay Wallet~\cite{copay-wallet}                                & $2 + (1/1)$        &                                                                       & N                                             & Y                                         & N                                                 & N                                                 & Y                                           & N                                                & P                                                      & Y                                                     & Y                                                   & A hybrid client-side wallet                                                          \\
			
			\midrule
			\smallskip
			\textbf{\specialcell{Split-Control --\\State-Aware Smart Contracts}} & $Z + (X_1/\ldots/X_z)$    &                                                                       &                                               &                                                         &                                                   &                                                   &                                             &                                                  &                                                        &                                                       &                                                      & \\
			\specialcell{TrezorMultisig2of3~\cite{TrezorMultisig2of3}}        & $2 + (1/1)$        & \specialcell{Assuming that each device\\is protected by a password}               & N                                             & Y                                                       & N                                                 & N                                                 & Y                                           & Y                                                & Y                                                      & Y                                                     & Y                                                                                &                                                                               \\
			Parity Wallet~\cite{parity-wallet}                               & $Z + (X_1/\ldots/X_z)$    & $Z$ is unlimited, $X_i$ = 1                                                & N                                             & Y                                                       & N                                                 & Y                                                 & Y                                           & N                                                & Y                                                      & Y                                                     & Y                                                    & \\
			Gnosis Wallet~\cite{ConsenSys-gnosis}                              & $Z + (X_1/\ldots/X_z)$    & $Z$ up to 50, $X_i$ = 1                                                    & N                                             & Y                                                       & N                                                 & Y                                                 & Y                                           & N                                                & Y                                                      & N/A                                                   & Y                                                    & \\
			\textbf{\textcolor{blue}{SmartOTPs}}                                        & $2 + (1/1)$        &  \specialcell{Private key and OTPs\\+ passwords}                                                                      & {Y}$^\circ$                                             & Y$^\$$                                                       & {Y}                                                 & Y                                                 & Y                                           & Y                                                & Y                                                      & Y                                                     & 						Y$^{\#}$    								& \specialcell{$^\circ$Fully air-gapped, if combined\\with ELLIPAL wallet\\  $^\$$Thanks to a hardware wallet\\$^{\#}$Also resilient to loss of all secrets} \\
			
			\midrule
			\smallskip
			\textbf{Server-Side Wallets}                         &   $0 + (X_1)$             &                                                                       &                                               &                                                         &                                                   &                                                   &                                             &                                                  &                                                        &                                                       &                                                      &                                      &                                                                               \\
			Coinbase~\cite{CoinbaseWallet}                                    & $0 + (2)$          &    Password, Google Auth./SMS                                                                    & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & N                                                      & Y                                                     & Y                                                    & \\
			Circle Pay~\cite{CircleWallet}                           & $0 + (2)$          & \dittoclosing                                                                      & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & N                                                      & Y                                                     & Y                                                    & \\
			Luno Wallet~\cite{luno-wallet}                                 & $0 + (2)$          &   Password and Google Auth.                                                                    & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & N                                                      & Y                                                     & Y                                                    & \\
			\midrule
			\textbf{Client-Side Wallets}                         &  $Z + (X_1)$          &                                                                       &                                               &                                                         &                                                   &                                                   &                                             &                                                  &                                                        &                                                       &                                                                                          &                                                                               \\
			Blockchain Wallet~\cite{BlockchainInfoWallet}                           & $1 + (2)$          &   \specialcell{Password and one of: Google\\Auth., YubiKey, SMS, or email}                                                                    & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & N                                                      & Y                                                     & Y                                                    &  \\
			BTC Wallet~\cite{BTC-com-wallet}                                  & $1 + (2)$          &        \dittoclosing                                 & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & N                                                      & Y                                                     & Y                                                    &  \\
			Mycelium Wallet~\cite{mycelium-wallet}                             & $1 + (1)$          &                                                                       & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & N                                                      & Y                                                     & Y                                                    &  \\
			CarbonWallet~\cite{CarbonWallet}                                & $2 + (2)$          &   \specialcell{2 private keys stored in\\browser and smartphone}                                                                    & N                                             & Y                                                       & N                                                 & N                                                 & N                                           & N                                                & N                                                      & Y                                                     & Y                                                    & \\
			Citowise Wallet~\cite{CitoWiseWallet}                             & $1 + (2)$          &                                                                       & N                                             & Y$^\P$                                                       & N                                                 & Y                                                 & N                                           & P$^\P$                                                & N                                                      & Y                                                     & Y                                                    &  \specialcell{$^\P$If combined with Trezor\\~or Ledger}               \\
			Coinomi Wallet~\cite{coinomi-wallet}                              & $1 + (1)$          &                                                                       & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & N                                                      & Y                                                     & Y                                                    & \\
			Infinito Wallet~\cite{InfinitoWallet}                              & $1 + (1)$          &                                                                       & N                                             & N                                                       & N                                                 & Y                                                 & N                                           & N                                                & N                                                      & Y                                                     & Y                                                    & 
			\\
			\bottomrule
		\end{tabular}
	}
	\caption{Comparison of state-of-the-art cryptocurrency wallets.}	
	\label{tab:state-of-the-art}
\end{table*}
\setlength{\tabcolsep}{1.4pt}
 


==> sec/wallet-types.tex <==
\subsection{Overview of Wallets}\label{appendix-soa}

\subsubsection{\textbf{Classification of Authentication Schemes}}\label{sec:classification}
\hfill

\noindent
We introduce the notion of $k$-factor authentication against the blockchain and $k$-factor authentication against the authentication factors.
Using these notions, we propose a classification of authentication schemes, and we apply it to examples of existing key management solutions (see \autoref{sec:soa-wallet-types} and \autoref{appendix:classification}).

In the context of the blockchain, we distinguish between k-factor authentication  \textit{against the blockchain} and k-factor authentication \textit{against the authentication factors} themselves.
For example, an authentication method may require the user to perform 2-of-2 multi-signature in order to execute a transfer, while $\mathbb{U}$ may keep each private key stored in a dedicated device -- each requiring a different password.
In this case, 2FA is performed against the blockchain, since both signatures are verified by all miners of the blockchain.
Additionally, a one-factor authentication is performed once in each device of $\mathbb{U}$ by entering a password in each of them.
For clarity, we classify authentication schemes by the following notation:
%
\begin{equation*}\label{eqn:auth-simple}
\Bigg ( 
Z 
+  X_1
\big/ \ldots \big/ 
X_Z
\Bigg),
\end{equation*}
where $Z \in \{0, 1, \ldots \}$ represents the number of authentication factors against the blockchain and
$X_i \in \{0, 1, \ldots \} ~|~i \in [1,\ldots, Z]$ represents the number of authentication factors against the i-th factor of $Z$.
%
With this in mind, we remark that the previous example provides $\left( 2 + 1/1 \right)$-factor authentication: twice against the blockchain (i.e., two signatures), once for accessing the first device (i.e., the first password), and once for accessing the second device (i.e., the second password).
%
Since the previous notation is insufficient for authentication schemes that use secret sharing~\cite{shamir1979share}, we
extend it as follows:
%
\begin{equation*}
\Bigg ( 
Z^{(W_1, \dots, W_Z)} 
+ \left( X_1^{1}, \ldots , X_1^{W_1} \right) 
\big/ \ldots \big/ 
\left(X_Z^{1}, \ldots, X_Z^{W_Z} \right) 
\Bigg),
\end{equation*}
%
where $Z$ has the same meaning as in the previous case, 
$W_i \in \{0, 1, \ldots \}$ $|~i \in [1,\ldots, Z]$ denotes the minimum number of secret shares required to use the complete i-th secret $X_i$.
%
%and
%$X_i^j \in \{0, 1, \ldots \} ~|~i \in [1,\ldots, Z], ~j \in [1,\ldots, W_i] $ represents the number of authentication factors against the i-th factor of $Z$, which, to be performed, additionally requires $W_i$ shares to use the full $i$th secret.
%
With this in mind, we remark that the aforementioned example provides $\left( 2^{(1, 1)} + (1)/(1) \right)$-factor authentication: twice against the blockchain (i.e., two signatures), once for accessing the first device (i.e., the first password), and once for accessing the second device (i.e., the second password).
We consider an implicit value of $W_i = 1$; hence, the classification $(2 + 1/1)$ represents the same as the previous one (the first notation suffices).
%
If one of the private keys were additionally split into two shares, each encrypted by a password, then such an approach would provide $\left( 2^{(2, 1)} + (1, 1)/(1) \right)$-factor authentication.
%\psz{Actually, what is value of this classification? We don't bind it to any properties nor try to give some metrics later on...}
%
%We remark that our solution belongs to the state aware smart contracts category and is most similar to~\cite{ConsenSys-gnosis} and~\cite{TrezorMultisig2of3}, \textcolor{red}{but in contrast to them, it provides a protection against MitMa targeting IPC~\cite{bui2018man} by a usable air-gapped setting, customizable security features, and a resilience to quantum computing attacks.}

\subsubsection{\textbf{Wallet Types}}\label{sec:soa-wallet-types}
\hfill

\noindent
We extend the previous work of Eskandari et al.~\cite{eskandari2018first} and Bonneau et al.~\cite{2015-Bitcoin-SOK}, by categorizing and reviewing a few examples of key management solutions.


\paragraph{\textbf{Keys in Local Storage}}
In this category of wallets, the private keys are stored in plaintext form on the local storage of a machine, thus providing $(1+0)$-factor authentication.
%
Examples that enable the use of unencrypted private key files are Bitcoin Core~\cite{BitcoinCore} or MyEtherWallet~\cite{MyEtherWallet} wallets.
%One disadvantage of this approach is that any process/user that has access to a directory that contains private keys can steal them. % (e.g., private-key-searching malware).


\paragraph{\textbf{Password-Protected Wallets}}
These wallets require the user-spe\-ci\-fied password to encrypt a private key stored on the local storage, thus providing $(1+1)$-factor authentication.
Examples that support this functionality are Armory Secure Wallet~\cite{Armory-SW-Wallet}, Electrum Wallet~\cite{Electrum-SW-Wallet}, MyEtherWallet~\cite{MyEtherWallet}, Bitcoin Core~\cite{BitcoinCore}, and Bitcoin Wallet~\cite{BitcoinWallet}.
%
This category addresses physical theft, yet enables the brute force  of passwords and digital theft (e.g., keylogger).
%In the case of digital theft, a keylogger can be installed on a device with keys.


\paragraph{\textbf{Password-Derived Wallets}}
% The original idea of password-deri\-ved wallets is attributed to Gregory Maxwell~\cite{maxwell2011deterministic}.
Password-derived wallets~\cite{maxwell2011deterministic} (a.k.a., brain wallets or hierarchical deterministic wallets) can compute a sequence of private keys from only a single mnemonic string and/or password.
This approach takes advantage of the key creation in the ECDSA signature scheme that is used by many blockchain platforms.
% Thanks to the homomorphism feature of discrete logarithm-based asymmetric crypto-systems, alike in the case of generating a sequence of private keys it is possible to deterministically generate a sequence of corresponding public keys based on a public mnemonic string, which has positive practical implications.
%
%Some password-derived wallets may enable $\mathbb{U}$ to select a short passphrase and then compute a longer seed by a key-stretching function (e.g., PBKDF2) serving for actual derivation of a key sequence~\cite{eskandari2018first}.
%However, such an approach provides a small entropy in seed computation; hence a brute force attack may reveal weak and short passwords.
%A more highly recommended method of seed computation in password-derived wallets is to let a wallet (pseudo-)randomly generate and encode a mnemonic with the length of $\geq$128 bits (e.g., by BIP-39~\cite{bipMnemonic}), and then compute a seed by a key stretching function (e.g., PBKDF2). 
%%
%Additionally, a user-specified passphrase (also referred to as seed extension) may be added to a seed computation as a salt in order to create (limited) protection against physical theft.
Examples of password-derived wallets are Electrum~\cite{Electrum-SW-Wallet}, Armory Secure Wallet~\cite{Armory-SW-Wallet}, Metamask~\cite{MetamaskWallet}, and Daedalus Wallet~\cite{daedalus-wallet}.
%
%A disadvantage of the example wallets of this category is that they do not enable to use MSA against the blockchain, only against accessing the wallet itself.
The wallets in this category provide $(1+X_1)$-factor authentication (usually $X_1 = 1$) and also suffer from weak passwords~\cite{courtois2016speed}.

%Moreover, the recent research also made advancements in the speedup of brute force attacks against brain wallets, which enabled to crack more complex passwords~\cite{courtois2016speed}.

%This category of wallets can be viewed as an extension of the password-derived wallets.
%Also, this category can be extended by further described categories of wallets. %, regardless they are self-sovereign or not.
%
%Thus far, all key management approaches did not provide a defense against a tampered client, as no 2FA or equivalent means was used.
%

\paragraph{\textbf{Hardware Storage Wallets}}
In general, wallets of this category include devices that can only sign transactions by private keys stored inside sealed storage, while the keys never leave the device. 
%
To sign a transaction, $\mathbb{U}$ connects the device to a machine and enters his passphrase.
%...either directly to a device using a touchscreen/keyboard or to an application running on a machine using a scrambled keyboard in order to prevent keyloggers.
When signing a transaction, the device displays the transaction's data to $\mathbb{U}$, who may verify the details. % in order to avoid confirmation of transaction crafted by a tampered client.
%
Thus, wallets of this category usually provide $(1+1)$-factor authentication.
%However, an attacker who has unauthorized full access to a device does not differ from an attacker that stole private keys~\cite{eskandari2018first}.
%Note that this category may be viewed as a special case of offline storage, and additionally, may have shared features of other categories (e.g., split control).
%
%
Popular USB (or Bluetooth) hardware wallets containing displays are offered by Trezor~\cite{trezor-hw-wallet},  Le\-dger~\cite{ledger-nano-s}, KeepKey~\cite{keep-key}, and BitLox~\cite{BitLox}.
%
An example of a USB wallet that is not resistant against tampering with $\mathbb{C}$ (e.g., keyloggers) is Ledger Nano~\cite{ledger-nano}
-- it does not have a display, hence $\mathbb{U}$ cannot verify the details of transactions being signed.
%and after connecting to a machine, it requires a user to enter a PIN code through $\mathbb{C}$ running on the machine.
%
An air-gapped transfer of transactions using QR codes is provided by ELLIPAL wallet~\cite{ellipal-hw-wallet}.
In ELLIPAL, both $\mathbb{C}$ (e.g., smartphone App) and the hardware wallet must be equipped with cameras and display.
$(1+0)$-factor authentication is provided by a credit-card-shaped hardware wallet from CoolBitX~\cite{CoolWalletS}. % The wallet communicates with a smartphone app by Bluetooth. 
%Also, Ledger Nano requires to enter validation code from $\mathbb{U}$'s grid card as the additional authentication factor, yielding $(1+2)$-factor authentication. 
%However, it does not help to defend against an attacker who tampers with $\mathbb{C}$ of the approach.% -- a user may be deceived and thinks that he executes one transaction, while attacker's transaction is executed.
%
%
A hybrid approach that relies on a server providing a relay for 2FA is offered by BitBox~\cite{BitBox}.
Although a BitBox device does not have a display, after connecting to a machine, it communicates with $\mathbb{C}$ running on the machine and at the same time, it communicates with a smartphone App through BitBox's server; 
each requested transaction is displayed and confirmed by $\mathbb{U}$ on the smartphone. 
%\done{Therefore, possession of a USB device, paired smartphone, and knowledge of a password to unlock a USB device yield $(1+2)$-factor authentication.}
%Hence, an attacker who tampers with $\mathbb{C}$ running at a machine is defended by a smartphone app.
%However, if this client is tampered with before setting up 2FA with a smartphone, an attacker may perform a MITM attack, which in turn will enable to display legitimate transaction data at user's smartphone, while the malicious transaction is being signed by a device.
One limitation of this solution is the lack of self-sovereignty.
%, as 2FA requires a connection to a server.
%



%
%From all of the mentioned devices only BitLox~\cite{BitLox} provides optional protection against the evil maid attack by introducing a secondary password for encryption of a user-specified phrase that must be decrypted and visually verified each time a user starts to use a device.
%\ih{Add new category of HW wallet using QR codes -- e.g., Ellipo, }

\paragraph{\textbf{Split Control -- Threshold Cryptography}}
In threshold cryptography~\cite{shamir1979share,threshold-mackenzie2001two,threshold-gennaro2007secure,blakley1979safeguarding}, a key is split into several parties which enables the spending of crypto-tokens only when n-of-m parties collaborate.
Threshold cryptography wallet provide $\left( 1^{(W_1, \ldots, W_n)}\- + (X_1, \dots, X_n) \right)$-factor authentication, as only a single signature verification is made on a blockchain, but $n$ verifications are made by parties that compute a signature.
Therefore, all the computations for co-signing a transaction are performed off-chain, which provides anonymity of access control policies (i.e., a transaction has a single signature) in contrast to the multi-signature scheme that is publicly visible on the blockchain.
%
An example of this category is presented by Goldfeder et al.~\cite{goldfeder2015securing}.
One limitation of this solution is a computational overhead that is directly proportional to the number of involved parties $m$ (e.g., for $m = 2$ it takes $13.26$s).
%
Another example of this category is a USB dongle called Mycelium Entropy~\cite{mycelium-entropy}, which, when connected to a printer, generates triplets of paper wallets using 2-of-3 Shamir's secret sharing; providing $(1^{(2)} + (0, ~0))$-factor authentication.

\paragraph{\textbf{Split Control -- Multi-Signature Wallets}}
In the case of multi-signature wallets, n-of-m owners of the wallet must co-sign the transaction made from the multi-owned address.
Thus, the wallets of this category provide $(n + X_1/\ldots/X_n)$-factor authentication.
One example of a multi-owned address approach is Bitcoin's Pay to Script Hash (P2SH).\footnote{We refer to the term  \textit{multi-owned address of P2SH} for clarity, although it can be viewed as Turing-incomplete smart contract.}
Examples supporting multi-owned addresses are Lockboxes of Armory Secure Wallet~\cite{Armory-SW-Wallet} and Electrum Wallet~\cite{Electrum-SW-Wallet}.
A property of multi-owned address is that each transaction with such an address requires off-chain communication. 
%(e.g., by email or instant messengers) and a confirmation of each transaction by the required number of owners.
%
A hybrid instance of this category and client-side hosted wallets category is Trusted Coin's cosigning service~\cite{TrustedCoin-cosign}, which provides a 2-of-3 multi-signature scheme -- $\mathbb{U}$ owns a primary and a backup key, while TrustedCoin owns the third key.
Each transaction is signed first by user's primary key and then, based on the correctness of the OTP from Google Authenticator, by TrustedCoin's key.
%
Another hybrid instance of this category and client-side hosted wallets is Copay Wallet~\cite{copay-wallet}.
With Copay, the user can create a multi-owned Copay wallet, where $\mathbb{U}$ has all keys in his machines and each transaction is co-signed by n-of-m keys.
Transactions are resent across user's machines during multi-signing through Copay.
%The advantage of this solution is that a user can view the details of a transaction when cosigning a transaction by each machine, which can defend $\mathbb{C}$ that is tampered with at one machine.
%This solution provides $(2+1/1)$-factor authentication.


\paragraph{\textbf{Split-Control -- State-Aware Smart Contracts}}\label{sec:state-aware=contracts}
State-aware smart contracts provide ``rules'' for how crypto-tokens of a contract can be spent by owners, while they keep the current setting of the rules on the blockchain.
%
The most common example of state-aware smart contracts is the 2-of-3 multi-signature scheme that provides $(2+X_1/X_2)$-factor authentication.
%Such a scheme is primarily intended for more users who share their crypto-tokens, but it can be also used in a user-sovereign fashion requiring a user to own all 3 accounts while keeping the keys at dedicated devices. 
%
An example of the 2-of-3 multi-signature approach that only supports Trezor hardware wallets is \textit{TrezorMultisig2of3} from Unchained Capital~\cite{TrezorMultisig2of3}.
%The advantages of this solution are its simplicity and independence from external libraries.
One disadvantage of this solution is that $\mathbb{U}$ has to own three Trezor devices, which may be an expensive solution that, moreover, relies only on a single vendor.
%
% I skipped BitGo~\cite{BitGo-MultiSigWallet}, which is also 2-of-3
%
Another example of this category, but using the n-of-m multi-signature scheme, is Parity Wallet~\cite{parity-wallet}. 
%Parity wallet enables several owners to independently confirm the requested operation of a smart contract. 
However, two critical bugs~\cite{parity-bug-July-17,parity-bug-November-17} have caused the multi-signature scheme to be currently disabled.
%
The n-of-m multi-signature scheme is also used in \textit{Gnosis Wallet} from ConsenSys~\cite{ConsenSys-gnosis}. %, further maintained under the Gnosis project~\cite{ConsenSys-gnosis}.
%The advantage of this solution is its integration with various kinds of software and hardware wallets, which enables the price-efficient combination of solutions from several vendors.

%
% which in the case of $\mathbb{A}$ is implemented as a smartphone app. 
%While $(2+2/1)$-factor authentication is provided in the case of $\mathbb{A}$ is implemented as a dedicated HW device, adding a secondary password for protection against the evil maid attacker.
%

%However in contrast to them, we are not limited to the multi-signature scheme, but we aim at the generalization of 2FA with necessary security guarantees against the wide scope of attacker models.
%In particular, we cover a defense against the tampered client, the evil maid attacker, and scamming of $\mathbb{A}$.




\paragraph{\textbf{Hosted  Wallets}}
Common features of hosted wallets are that they provide an online interface for interaction with the blockchain, managing crypto-tokens, and viewing transaction history, while they also store private keys at the server side.
If a hosted wallet has full control over private keys, it is referred to as a \textit{server-side wallet}. 
A server-side wallet acts like a bank -- the trust is centralized.
Due to several cases of compromising such server-side wallets~\cite{2018-coindesk-bithumb}, \cite{2014-Mt-Gox}, \cite{2016-Bitfinex-hack}, \cite{moore2013beware}, the hosted wallets that provide only an interface for interaction with the blockchain (or store only user-encrypted private keys) have started to proliferate.
In such wallets, the functionality, including the storage of private keys, has moved to $\mathbb{U}$'s browser (i.e., client).
We refer to these kinds of wallets as \textit{client-side wallets} (a.k.a., hybrid wallets~\cite{eskandari2018first}).

\paragraph{\textbf{Server-Side Wallets}}
Coinbase~\cite{CoinbaseWallet} is an example of a server-side hosted wallet, which also provides exchange services.
Whenever the user logs in or performs an operation, he authenticates himself against Coinbase's server using a password and obtains a code from Google Authenticator/Authy app/SMS. 
%However, no transaction data are verified by 2FA method, which creates an opportunity for an attacker that tampers with $\mathbb{C}$ in a way that user is tricked to confirm a legitimate transaction, while attacker's transaction is confirmed.
%Another attack vector exists during installation of 2FA when $\mathbb{C}$ is already tampered with -- stealing of shared secret of Google Authenticator enables to replicate it.
%
Other examples of server-side wallets having equivalent security level to Coinbase are Circle Pay Wallet~\cite{CircleWallet} and Luno Wallet~\cite{luno-wallet}.
The wallets in this category provide $(0+2)$-factor authentication when 2FA is enabled.


\paragraph{\textbf{Client-Side Wallets}}
%\todo{(X+Y) here}
An example of a client-side hosted wallet is Blockchain Wallet~\cite{BlockchainInfoWallet}. 
Blockchain Wallet is a password-derived wallet that provides 1-factor authentication against the server based on the knowledge of a password and additionally enables 2FA against the server through one of the options consisting of Google Authenticator, YubiKey, SMS, and email.
%However, the 2FA serves only for login purposes to an online website, not for confirmation of a transaction.
When creating a transaction, $\mathbb{U}$ can be authenticated by entering his secondary password. %, but again no transaction data are authenticated. 
%Overall, the wallet provides $(1+2)$-factor authentication.
%Since Blockchain wallet is password-derived only from a user's passphrase, in the case of tampered client or DNS spoofing attack or key logging malware, an attacker may grasp user's crypto-tokens by simply extracting a main password from a user during a login attempt to a tampered client, a spoofed URL, or an original client, respectively.
%
Equivalent functionality and security level as in Blockchain Wallet are offered by BTC Wallet~\cite{BTC-com-wallet}. % (formerly known as Blocktrail Wallet).
In contrast to Blockchain Wallet, BTC wallet uses 2FA also during the confirmation of a transaction. 
%However, similarly no transaction data are authenticated by 2FA.
%
Other examples of this category are password-derived wallets, like Mycelium Wallet~\cite{mycelium-wallet}, CarbonWallet~\cite{CarbonWallet}, Citowise Wallet~\cite{CitoWiseWallet}, Coinomi Wallet~\cite{coinomi-wallet}, and Infinito Wallet~\cite{InfinitoWallet}, which, in contrast to the previous examples, do not store backups of encrypted keys at the server.
A 2FA feature is provided additionally to password-based authentication, in the case of CarbonWallet.
In detail, the 2-of-2 multi-signature scheme uses the machine's browser and the smartphone's browser (or the app) to co-sign transactions. % that are delivered to a smartphone via a CarbonWallet server.
% while private keys are stored encrypted in a machine's browser and a smartphone's browser/application, respectively.
%
% In contrast to Blockchain and BTC wallets, CarbonWallet has smaller attack surface of a tampered client in machine's browser.
% In detail, if $\mathbb{C}$ in browser is tampered with when a user performs a registration, an attacker may trick a user to use malicious URL or scam application in user's smart phone during installation of 2FA. \feedback{Check it again.}
%
%\feedback{Evaluate our approach according to framework in Table I of \cite{eskandari2018first}.}


%\paragraph{Notes after review from NDSS}
%An observation is that T/Key~\cite{kogan2017t} is using time-constrained OTPs to make ``phishing attacks more difficult because the attacker has a limited time window in which to use the stolen password.'' 
%SmartOTPs protects against such an attack by protocol with 2 stages. 
%Moreover, thanks to invalidation of layers in hash chains, the old OTPs are no longer valid, which emulates the time boundaries of T/Key. 
%\ih{check different hash functions and salting to protect birthday and preprocessing attacks, respectively}






